From Hard to Soft: Understanding Deep Network Nonlinearities via Vector Quantization and Statistical Inference

Nonlinearity is crucial to the performance of a deep (neural) network (DN). To date there has been little progress understanding the menagerie of available nonlinearities, but recently progress has been made on understanding the r\^ole played by piecewise affine and convex nonlinearities like the ReLU and absolute value activation functions and max-pooling. In particular, DN layers constructed from these operations can be interpreted as {\em max-affine spline operators} (MASOs) that have an elegant link to vector quantization (VQ) and $K$-means. While this is good theoretical progress, the entire MASO approach is predicated on the requirement that the nonlinearities be piecewise affine and convex, which precludes important activation functions like the sigmoid, hyperbolic tangent, and softmax. {\em This paper extends the MASO framework to these and an infinitely large class of new nonlinearities by linking deterministic MASOs with probabilistic Gaussian Mixture Models (GMMs).} We show that, under a GMM, piecewise affine, convex nonlinearities like ReLU, absolute value, and max-pooling can be interpreted as solutions to certain natural "hard" VQ inference problems, while sigmoid, hyperbolic tangent, and softmax can be interpreted as solutions to corresponding "soft" VQ inference problems. We further extend the framework by hybridizing the hard and soft VQ optimizations to create a $\beta$-VQ inference that interpolates between hard, soft, and linear VQ inference. A prime example of a $\beta$-VQ DN nonlinearity is the {\em swish} nonlinearity, which offers state-of-the-art performance in a range of computer vision tasks but was developed ad hoc by experimentation. Finally, we validate with experiments an important assertion of our theory, namely that DN performance can be significantly improved by enforcing orthogonality in its linear filters.

==> adversarial.tex <==
\section{Adversarial Examples}
We propose to study in this section adversarial noise made from the gradient of of the mapping wrong class prediction w.r.t. the input.

By definition, the adversarial noise is created by combination of the class representation $W^{(L)}_c$ and the input features $\bz^{(L-1)}$. Based on this, the noise simply corresponds to the DN representation of the input with the wrong class. 
\begin{prop}
Such adversarial noise between class $c_1$ and $c_2$ can only exist if $||\sum_{d} W_{c_1,d}\frac{d \bz^{(L-1)}_{d}[x_{c_1}]}{dx_{c_1}} || > 0$.
\end{prop}

While this provides a principled way to prevent adversarial noise, we now propose further experiments to understand what happens in the DN.
We will demonstrate that aadversarial noise comes from :
\begin{itemize}
\item Shared Features accross classes
\item high norm of the weights
\item high sensitivity of the region w.r.t. noise (due to small sized filters)
\end{itemize}

The first one amplifies the sensitivity as it pushes the noise not just to increase
Removing the bias !
Is it better ?








==> background.tex <==
\section{Background on Deep Networks}
\label{sec:back}

%Regardless of the network topology,
A deep network (DN) is an operator $f_\Theta: \R^D \rightarrow \R^C$ that maps an input signal
$\bx\in\R^D$ to an output prediction $\widehat{y} \in \R^C$ as $f_\Theta: \R^D \rightarrow \R^C$.
All current DNs can be written as a  composition of $L$ intermediate mappings called {\em layers}
\begin{equation}
%\widehat{y}=
f_\Theta(\bx)= \left(f^{(L)}_{\theta^{(L)}} \circ \dots \circ f^{(1)}_{\theta^{(1)}}\right)\!(\bx),
\label{eq:layers1}
\end{equation}
where $\Theta=\left\{\theta^{(1)},\dots,\theta^{(L)}\right\}$ is the 
collection of the network's parameters from each layer.
This composition of mappings is nonlinear and non-commutative, in general.

The DN {\em layer} at level $\ell$ is an operator $f^{(\ell)}_{\theta^{(\ell)}}$ that takes as input the vector-valued signal $\bz^{(\ell-1)}(\bx)\in \R^{D^{(\ell-1)}}$ and produces the vector-valued output $\bz^{(\ell)}(\bx)\in \R^{D^{(\ell)}}$ with $D^{(L)}=C$. 
The signals $\bz^{(\ell)}(\bx),\ell \geq 1$ are typically called {\em feature maps}; it is easy to see that \roro{trivial so it is useless in my opinion}
\begin{equation}
\bz^{(\ell)}(\bx)=\left(f^{(\ell)}_{\theta^{(\ell)}} \circ \dots \circ f^{(1)}_{\theta^{(1)}}\right)\!(\bx),~~\ell \in \{1,\dots,L\}
\label{eq:layers2}
\end{equation}
%
with the initialization $\bz^{(0)}(x):=x$ and $D^{(0)}:=D$.


For concreteness, we focus here on processing multichannel images $x$, \roro{previous is enough, everybody know that images are  RGB} such as RGB color digital photographs.
However, our analysis and techniques apply to signals of any index-dimensionality, including speech and audio signals, video signals, etc., simply by adjusting the appropriate dimensionalities.
%



For sake of clarity, we will propose two conventions: the first one will be based on tensors notation for both the input signal $x$ and the inner representation $z^{(\ell)}$ of the DN, while the second one will be its flattened version leading to vector notation $\bx$ and $\bz^{(\ell)}$.
In the vector representation, 
$[\bx]_d$ represents the entry of the $d^{\rm th}$ dimension of the flattened version of $x$.
In the tensor representation, the input image $x$ contains $C^{(0)}$ channels of size $I^{(0)} \times J^{(0)}$ pixels, and the feature map $z^{(\ell)}$ contains $C^{(\ell)}$ channels of size $(I^{(\ell)} \times J^{(\ell)})$ pixels.
Hence, $D^{(\ell)}=C^{(\ell)}I^{(\ell)}J^{(\ell)}$, 
$C^{(L)}=C$, $I^{(L)}=1$, and $J^{(L)}=1$.


We briefly overview the basic DN operators and layers we consider in this paper; more details and additional layers can be found in \cite{goodfellow2016deep}  (\roro{citing Goodfellow? why? I guess there are other refs that are better and less about hype and trend about the fancy new book of the new star crowned by our favorite dictator Yann Le Cun})
and the SM. 


A \textbf{{\em fully connected operator}} performs an arbitrary affine transformation by multiplying its input by the dense matrix $\bW^{(\ell)} \in \mathbb{R}^{D^{(\ell)} \times D^{(\ell-1)}}$ and adding the arbitrary bias vector $\bb_\bW^{(\ell)} \in \mathbb{R}^{D^{(\ell)}}$, as in $f^{(\ell)}_\bW \!\left(\bz^{(\ell-1)}(\bx)\right):=   \bW^{(\ell)}\bz^{(\ell-1)}(\bx)+\bb_\bW^{(\ell)}$.


A \textbf{{\em convolution operator}} performs a constrained affine transformation on its input by multiplying by the multichannel block circulant convolution matrix $\bC^{(\ell)}\in \mathbb{R}^{D^{(\ell)} \times D^{(\ell-1)}}$ and adding the bias vector $\bb_{\bC}^{(\ell)} \in \mathbb{R}^{D^{(\ell)}}$, as in $f^{(\ell)}_{\bC} \!\left(\bz^{(\ell-1)}(\bx)\right):= \bC^{(\ell)}\bz^{(\ell-1)}(\bx)+\bb_{\bC}^{(\ell)}$.
%
The multichannel convolution matrix applies $C^{(\ell)}$ different filters of dimension $(C^{(\ell-1)},I^{(\ell)}_{\bC},J^{(\ell)}_{\bC})$ to the input. Thus each filter is a $C^{(\ell-1)}$-channel filter of spatial size $\left(I^{(\ell)}_{\bC},J^{(\ell)}_{\bC}\right)$.
%
In addition, the bias $\bb_{\bC}^{(\ell)}$ is constrained to be (potentially different) constant for each of the $C^{(\ell)}$ output channels.  
%
The convolution and bias constraints radically reduce the number of parameters as compared to a fully connected operator but impose a structural bias of translation invariance \cite{lecun1998mnist}.  
%In fact, the number of degrees of freedom of $\bC$ is $C^{(\ell)}M^{(\ell)}N^{(\ell)}$ with $(M^{(\ell)}m^{(\ell)})$ the spatial size of the filters. 
%The bias contains $C^{(\ell)}$ degrees of freedom. 
%
%Without diving into details on boundary conditions and padding for this operator, the output dimension is thus defined as $D^{(\ell)}=C^{(\ell)}I^{(\ell-1)}J^{(\ell-1)}$ hence maintaining same spatial dimension.
%
Additional details are provided in the SM.


An \textbf{{\em activation operator}} applies a scalar nonlinear {\em activation function} $\sigma$ separately to each entry of its input\roro{shorter: a point-wise nonlinearity}, as in $
    [f^{(\ell)}_\sigma \!\left(\bz^{(\ell-1)}(\bx)\right)]_k=\sigma\! \left([\bz^{(\ell-1)}(\bx)]_k\right)$, $k=1,\dots,D^{(\ell)}$.
Nonlinearities are crucial to DNs, since otherwise the entire network would collapse to a single global affine transform. 
Generally, a different nonlinearity can be used for each dimension of $\bz^{(\ell-1)}(\bx)$, but today's standard practice employs the same $\sigma$ across all entries.
Three popular activation functions are the {\em rectified linear unit} (ReLU)
$\sigma_{\rm ReLU}(u):=\max(u,0)$, the {\em leaky ReLU}
$\sigma_{\rm LReLU}(u):= \max(\eta u,u),\;\eta>0$, and the {\em absolute value} $\sigma_{\rm abs}(u):=|u|$.
These three functions are both piecewise affine and convex.
Other popular activation functions include the {\em sigmoid} $\sigma_{\rm sig}(u):=\frac{1}{1+e^{-u}}$ and
{\em hyperbolic tangent} $\sigma_{\rm tanh}(u):=2\sigma_{\rm sig}(2u)-1$.
These two functions are neither piecewise affine nor convex.

%We will emphasize nonlinearities that are both piecewise linear and convex in this paper; these include the {\em rectified linear unit} (ReLU),
%the {\em leaky ReLU} and the {\em absolute value}.
%Additional nonlinearities that are neither piecewise linear nor convex include the sigmoid and hyperbolic tangent.

A \textbf{{\em pooling operator}} subsamples its input to reduce its dimensionality according to a sub-sampling policy $\rho$ applied over $K^{(\ell)}$ pooling regions defined by the collection of indices
$\left\{\mathcal{R}^{(\ell)}_k\right\}_{k=1}^{K^{(\ell)}}$. 
Pooling regions typically correspond to small, non-overlapping image blocks or channel slices. 
A widely used policy $\rho$ is {\em max-pooling} $
    [f^{(\ell)}_\rho \! \left(\bz^{(\ell-1)}(\bx)\right)]_k
    =
    \max_{i\in \mathcal{R}^{(\ell)}_k} [\bz^{(\ell-1)}(\bx)]_i ,d=1,\dots,D^{(\ell)}$. 
%The collection of indices $\mathcal{R}_k$ thus correspond to the positions on the input onto which the pooling policy $\rho$ is applied, typically small patches in DNs.
See the SM for the precise definition plus the definition of {\em average pooling} and {\em channel pooling}, which is used in maxout networks \cite{goodfellow2013maxout}.


See the SM \roro{see the SM, see the SM, see the SM... I guess they can understand that since you mentioned it at the beginning of the section} for the definition of the operators corresponding to the {\em skip connections} used in skip connection networks \cite{srivastava2015training} and residual networks (resnets) \cite{resnet-he,targ2016resnet} and the {\em recurrent connections} used in RNNs \cite{graves2013generating}.

For the purposes of this paper, we will use the following definition of a layer.

%For example, standard terminology associates a convolutional layer to a convolution operator followed by activation operator. 
%A DN layer consists of a composition of any of the above operators. 
%such that there is one nonlinear operator (nonlinearity or pooling) in order to ease the notations below.
%For example, the classical CNN layer consists of convolution followed by activation and pooling.

\begin{defn}
A DN {\em layer} $f^{(\ell)}$ comprises a single nonlinear DN operator composed with any (if any) preceding linear operators that lie between it and the preceding nonlinear operator.
\label{def:layer}
\end{defn}
\qq

This definition yields a single, unique layer decomposition of any DN, and the complete DN is then the composition of its layers per (\ref{eq:layers1}). 
For example, in a standard CNN, there are two different layers types: i) convolution followed by activation and ii) max-pooling.
%For another example, a skip-connection operator that skips around a convolution operator followed by an activation operator corresponds to a single layer.

\textbf{Output Layer}
%\roro{maybe using the same format: \textbf{Output Layer}}
The final layers in a DN typically consist of one or more fully connected operators interspersed with activation operators.  
We form the prediction by feeding the DN output $f_\Theta(\bx)$ through a final nonlinearity $g:\mathbb{R}^{C}\rightarrow \mathbb{R}^{C}$ to form $\widehat{y}=g(f_\Theta(\bx))$.
For classification problems, $g$ is typically the {\em softmax}, which arises naturally from posing the classification inference as a multinomial logistic regression problem \cite{bishop1995neural}.
Other options are available, such as the {\em spherical softmax} \cite{de2015exploration}.
See the SM for the definition.
%Another example is the {\em spherical softmax} \cite{de2015exploration}.
%and the last operator of the DN is a fully connected one.
For regression problems, typically no $g$ is applied. 

\iffalse
Given an input signal $x$, the DN computes the prediction via  $\widehat{y}=z=f_\Theta(x)$ or $\widehat{y}=g(z)=g(f_\Theta(x))$ depending on the application.  
%
For regression problems, the prediction $\widehat{y}$ should be continuous-valued, and thus the DN usually contains a linear last layer and the output $z$ is taken as the prediction.
%
For classification problems, the prediction $\widehat{y}$ should be categorical, and thus the DN output $z$ is typically processed through a nonlinear function $g$ that converts it into a probability density over $c$ that represents 
$\mathbb{P}(\text{class of $x$ is $c$}\:|\:x)$. 
The preeminent example is the {\em softmax nonlinearity} 
that arises naturally from posing the classification inference as a multinomial logistic regression problem \cite{bishop1995neural}.
Another example is .
\fi 

%\roro{maybe using the same format: \textbf{Learning}}
\textbf{Learning}
We {\em learn} the DN parameters $\Theta$ for a particular prediction task in a supervised setting using a labeled data set $\mathcal{D}=(x_n,y_n)_{n=1}^N$,
a loss function, $\mathcal{L}:\mathbb{R}^{C} \times \mathbb{R}^{C} \rightarrow \mathbb{R}^+$, 
and a learning policy to update the parameters $\Theta$ in the predictor $f_\Theta(x)$.
%
For a $C$-class classification problem posed as a multinomial logistic regression \cite{bishop1995neural}, $y_n \in \{1,\dots,C\}$, and the loss function is typically the negative cross-entropy \roro{trivial and known so is it useful to write it here?}\randall{good point}
\begin{align}
    \mathcal{L}_{\rm CE}&(y_n,g(f_\Theta(\bx_n))) = -\log \left( [g(f_\Theta(\bx_n))]_{y_n}\right)\nonumber \\
    &= -[f_\Theta(\bx_n)]_{y_n}+\log\left(\sum_{c=1}^C e^{[f_\Theta(\bx_n)]_{c}}\right).
    \label{eq:crossEnt}
\end{align}
The total loss is obtained by summing over all of the $N$ samples in $\mathcal{D}$ or batches sampled from it.
%with target a categorical variable $y_n \in \{1,\dots,C\}$.
For regression problems, $y_n \in \mathbb{R}^C$, and the loss function is typically the mean squared error.
%
%As with regression, this is multiconvex function to optimize.
%
Since the layer-by-layer operations in a DN are differentiable almost everywhere with respect to their parameters and inputs, 
we can use some flavor of first-order optimization such as gradient descent to optimize the parameters $\Theta$ with respect to the loss.
Moreover, the gradients for all internal parameters can be computed efficiently using {\em backpropagation} \cite{hecht1988theory}, which follows from the chain rule of calculus. 
%leading to a computational complexity similar to the one of the forward pass.



==> deepMaso.tex <==
\section{Deep Networks are Compositions of Spline Operators}
\label{sec:deepMaso}

%\green{rewrite MASO to represent DN operator and derive properties}

A key result of this paper is that 
a large class of DNs can be written as a composition of MASOs, one for each layer.
This includes many standard DNs topologies, including CNNs, resnets, inception networks, maxout networks, network-in-networks, scattering networks, RNNs, and their variants.
To build such results, we first proceed by adapting MASOs for DN operators. Based on this rewritting, precise analysis of DN made of composition of MASO can be done. 
A composition of MASOs is non-convex in general and hence can approximate a much larger class of functions/operators.
Interestingly, under certain broad conditions, the composition remains a piecewise affine spline operator, which enables a variety of insights into DNs.

We now state our main theoretical results bridging DNs and MASOs with the proofs contained in Appendix~\ref{sec:proofs}. 

\subsection{DN Operators and Layers are MASOs}


We begin by showing that DN operators are MASOs.% in the SM.

\begin{prop}
An arbitrary fully connected operator $f^{(\ell)}_\bW$ is an affine mapping and hence a degenerate MASO $S\!\left[A_\bW^{(\ell)},B_\bW^{(\ell)}\right]$, with $R=1$, $[A^{(\ell)}_{\bW}]_{k,1,.}=\left[\bW^{(\ell)}\right]_{k,.}$, and $[B^{(\ell)}_{\bW}]_{k,1}=\left[\bb_{\bW}^{(\ell)}\right]_k$, leading to 
\begin{align}
& \bW^{(\ell)}\bz^{(\ell-1)}(\bx)+b_\bW^{(\ell)} = A_\bW^{(\ell)}[\bx]\bz^{(\ell-1)}(\bx)+B_\bW^{(\ell)}[\bx].
\end{align}
The same is true of a convolution operator with $\bW^{(\ell)},\bb_\bW^{(\ell)}$ replaced by $\bC^{(\ell)},\bb_{\bC}^{(\ell)}$.
\label{thm:conv}
\end{prop}
\begin{prop}
Any activation operator $f_\sigma^{(\ell)}$ using a piecewise affine and convex activation function is a MASO denoted by $S\!\left[\bA_\sigma^{(\ell)},\bB_\sigma^{(\ell)}\right]$. 
In particular, ReLU, leaky ReLU, and absolute value are MASOs with $R=2$,  $[\bB^{(\ell)}_\sigma]_{k,1}=[\bB^{(\ell)}_\sigma]_{k,2}=0,\forall k$ and  (ReLU:)$[\bA^{(\ell)}_\sigma]_{k,1,.}=0,[\bA^{(\ell)}_\sigma]_{k,2,.}=\be_k,\forall k$; (leaky ReLU:)  
$[\bA^{(\ell)}_\sigma]_{k,1,.}=\nu \be_k,[\bA^{(\ell)}_\sigma]_{k,2,.}=\be_k,\forall k,\nu>0$; and (absolute value:) $[\bA^{(\ell)}_\sigma]_{k,1,.}=-\be_k,[\bA^{(\ell)}_\sigma]_{k,2,.}=\be_k,\forall k$ .
(Here, $\be_k$ represents the $k^{\rm th}$ canonical basis element of $\mathbb{R}^{D^{(\ell)}}$.)
\label{thm:act}
\end{prop}
%\qq
%We introduce $\be_k$, as the output of an activation operator at index $k$ is dependent only on the input at the same index $k$; that is,
% $f_\sigma\left(\bz^{(\ell)}(\bx)\right)_k=\sigma\left([\bz^{(\ell)}(\bx)]_k\right)=\sigma\left(\langle \bz^{(\ell)}(\bx), \be_k \rangle\right)$.


\begin{prop}
Any pooling operator $f_\rho^{(\ell)}$ that is piecewise-affine and convex is a MASO denoted as $S\!\left[\bA^{(\ell)}_\rho,\bB^{(\ell)}_\rho\right]$.\footnote
{
This result is agnostic of the type of pooling (spatial or channel).
% as those details only change the indices present in $\mathcal{R}_k$. Details about those different pooling
Details are provided in Figure~\ref{fig:pooling} in Appendix XXXX.
}
Max-pooling has $R=\#\mathcal{R}_k$ (typically a constant over $k$), 
$[\bA^{(\ell)}_\rho]_{k,.,.}=\{ \be_{i},i \in \mathcal{R}_k\}$, 
and $ [\bB^{(\ell)}_\rho]_{k,r}=0,\forall k,r$.
Average-pooling is a degenerate MASO with $R=1$, 
$[\bA^{(\ell)}_\rho]_{k,1,.}=\frac{1}{\#(\mathcal{R}_k)}\sum_{i \in \mathcal{R}_k} \be_i$, and 
$[\bB^{(\ell)}_\rho]_{k,1}=0,\forall k$. 
\label{thm:pool}
\end{prop}
\qq
%The preceding propositions demonstrate how standard DNs operators are MASOs. This enables us to develop general results for DNs.


\iffalse

Recall our precise definition of a DN layer in Definition \ref{def:layer}.
%that was comprising (possibly multiple) MASOs (\ref{thm:act},\ref{thm:conv},\ref{thm:pool}).

\begin{prop}
A DN layer as defined in Def. \ref{def:layer} consisting of possibly multiple MASOs can be rewritten as a unique MASO.
\label{thm:layerMaso}
\end{prop}
\qq

This is natural as composition of a linear transformation such as a convolutional operator followed by a MASO operator such as nonlinearity or pooling is itself a MASO with modified parameters. Denote the layer-$\ell$ MASO slope and offset parameters (recall (\ref{eq:ASO})) by $S[\bA,\bB]^{(\ell)}$,notice the absence of subscript differentiating the MASO of a DN operator and  one of the whole layer..
\begin{defn}
As a result, we can now denote explicitly 
\begin{align}
    f^{(\ell)}(&\bz^{(\ell-1)}(\bx))=A^{(\ell)}[\bx]\bz^{(\ell-1)}(\bx)+B^{(\ell)}[\bx]
\label{eq:masopixel}
\end{align}
\end{defn}

%For sake of clarity we develop some results for MASO operator but hold for the more general ASO operators.
%We demonstrate before that any linear operator can be seen as a degenerate MASO with $R=1$.

An alternate interpretation of (\ref{eq:CNNaffine1}) leverages such simplification. This will highlight that $\bz_{\rm CNN}^{(L)}(\bx)$ is the output of a bank of linear {\em matched filters} (plus a set of biases).
That is, the $c^{\rm th}$ element of $\bz_{\rm CNN}^{(L)}(\bx)$ equals the inner product between the signal $x$ and the matched filter for the $c^{\rm th}$ class, which is contained in the $c^{\rm th}$ row of the matrix $\bW^{(L)}A_{\rm CNN}[\bx]$.
The bias $\bb^{(\ell)}$ can be used to account for the fact that some classes might be more likely than others (i.e., the prior probability over the classes). On the other hand, $\bW^{(L)}\bb_{\rm CNN}[\bx]$ is the induced bias from the induced MASO activations.
It is well-known that a matched filterbank is the optimal classifier for deterministic signals in additive white Gaussian noise \cite{rabiner1975theory}.
Given an input $\bx$, the class decision is simply the index of the largest element of $\bz_{\rm CNN}^{(L)}(\bx)$.\footnote
{Again, since the softmax merely rescales the entries of $\bz_{\rm CNN}^{(L)}(\bx)$ into a probability distribution, it does not affect the location of its largest element.}

\fi 


Combinations of DN operators that result in a layer (recall Definition~\ref{def:layer}) are also MASOs.


\begin{prop}
\label{thm:layerMASO}
A DN layer (recall Def. \ref{def:layer}) constructed from an arbitrary composition of fully connected/convolution operators of the type stated in Prop.~\ref{thm:conv} and one activation or pooling operator as stated in Prop.~\ref{thm:pool} is a MASO denoted as $S[A^{(\ell)},B^{(\ell)}]$ leading to
\begin{equation}
    f^{(\ell)}(\bz^{(\ell-1)})=A^{(\ell)}[\bx]\bz^{(\ell-1)}(\bx)+B^{(\ell)}[\bx].
    \label{eq:masopixel}
\end{equation}
\end{prop}
 For example, a layer composed of an activation operator ($S\!\left[\bA^{(\ell)}_\sigma,\bB^{(\ell)}_\sigma \right]$) and an affine transform ($S\!\left[\bA^{(\ell)}_\bW,\bB^{(\ell)}_\bW \right]$) is a MASO  $S\!\left[\bA^{(\ell)},\bB^{(\ell)}\right](\bz^{(\ell-1)}(\bx))$ with parameters $[\bA^{(\ell)}]_{k,r,.}=\bW^{(\ell)T}[\bA^{(\ell)}_\sigma]_{k,r,.}$ and $[\bB^{(\ell)}]_{k,r}=[\bB^{(\ell)}_\sigma]_{k,r}+\langle [\bA^{(\ell)}_\sigma]_{k,r},\bb_{\bW}^{(\ell)}\rangle $. More examples are provided in the SM.
We propose in the SM many examples on how to rewrite a composition of multiple DN operators/MASOS are one MASO representing the layer mapping in Sec.~\ref{sec:proof_rewritting}.
%Details are provided in the SM.
%Here are two simple examples.
%An affine transform followed by a MASO remains a MASO with new parameters.

% this is not needed
%\begin{prop}\label{composition}
%Any MASO following an affine transformation can be computed via definition of a new reparametrized MASO with $\textbf{h}_k=\{ \bW^T\ba_{k,r},\forall k,r \}$ and $\textbf{b}'=\{b_{k,\omega_r}+\bb^T\ba_{k,\omega_r},\forall k,r\}$ and $\mathcal{A}_k=\cup_{d \in \mathcal{A}_k}\mathcal{A}_d$.
%\end{prop}



\begin{figure*}[!t]
% ensure that we have normalsize text
\normalsize
% Store the current equation number.
%\setcounter{MYtempeqncnt}{\value{equation}}
% Set the equation number to one less than the one
% desired for the first equation here.
% The value here will have to changed if equations
% are added or removed prior to the place these
% equations are referenced in the main text.
%\setcounter{equation}{5}
\begin{align}
    \bz_{\rm CNN}^{(L)}(\bx) &= %\underbrace{
    \bW^{(L)}
    \underbrace{\left(
    \prod_{\ell=L-1}^1 A_{\rho}^{(\ell)}[\bx] A^{(\ell)}_{\sigma}[\bx] \bC^{(\ell)} \right)}_{A_{\rm CNN}[\bx]}
    %}_{\text{Linear}} 
    \bx+\bW^{(L)}\underbrace{
    %\underbrace{
    \sum_{\ell=1}^{L-1}
    \left(
    \prod_{j=L-1}^{\ell+1}A_{\rho}^{(j)}[\bx]
    A^{(j)}_{\sigma}[\bx] \bC^{(j)}
    \right)\!
    \left(A_{\rho}^{(\ell)}[\bx]
    A^{(\ell)}_{\sigma}[\bx] \bb_{\bC}^{(\ell)}
    \right)}_{\bb_{\rm CNN}[\bx]}+\bb_{\bW}^{(L)}
    %}_{\text{Offset}}
    \label{eq:CNNaffine}
%    \\
%    &= W^{(L)}
%    \underbrace{\left[ \left(
%    \prod_{\ell=L-1}^1 A_{\rho}^{(\ell)} A^{(\ell)}_{\sigma} \bC^{(\ell)} \right) x+\sum_{\ell=1}^{L-1}
%    \left(
%    \prod_{j=L-1}^{\ell+1}A_{\rho}^{(j)}A^{(j)}_{\sigma} \bC^{(j)}
%    \right)\!
%    \left(A_{\rho}^{(\ell)}A^{(\ell)}_{\sigma} b^{(\ell)}
%    \right)\right]}_{\text{Pre-Processing}}+b^{(L)}.
%    \label{eq:zCNN}
\end{align}
% Restore the current equation number.
%\setcounter{equation}{\value{MYtempeqncnt}}
% IEEE uses as a separator
%\hrulefill
% The spacer can be tweaked to stop underfull vboxes.
%\vspace*{4pt}
%\hline 
\normalsize
\vspace*{-10mm}
\end{figure*}

\subsection{Compositions of MASOs}

We first propose the following lemma to ease the following general results about DNs.
\begin{lemma}
\label{thm:lemma1}
A composition of multiple MASOs with parameters $A^{(l)},B^{(l)},l=1,\dots,L$ is always an ASO.
\end{lemma}
Based on the previous lemma, we can now state results about the functional form of DNs composed of MASO operators.
\begin{theorem}
Based on Lemma \ref{thm:lemma1} and Prop.~\ref{thm:layerMASO}, a DN constructed from an arbitrary composition of layers from Proposition~\ref{thm:layerMASO} is an ASO.
\label{thm:big2}
\end{theorem}
\qq
\roro{maybe put the next "example" as a proposition or a remark}
DNs covered by Theorem \ref{thm:big2} include CNNs, resnets, inception networks, maxout networks, network-in-networks, scattering networks, and their variants using connected/convolution operators, (leaky) ReLU or absolute value activations, and max/mean pooling. 


Note carefully that, DNs of the form stated in Theorem \ref{thm:big2} are not MASOs, in general, since the composition of two or more MASOs is not necessarily a MASO.
Indeed, a composition of MASOs remains a MASO if and only if all of the intermediate operators are non-decreasing with respect to each of their output dimensions \cite{boyd2004convex}.
Interestingly, ReLU, max-pooling, and average pooling are all non-decreasing, while Leaky-ReLU is strictly increasing. 
The culprits of the non-convexity of the composition of operators are negative entries in the fully connected and convolution operators.
A DN where these culprits are thwarted is an interesting special case, because it will be convex with respect to the input \cite{amos2016input} and multiconvex \cite{xu2013block} with respect to the parameters (i.e., convex with respect to each operator's parameters while the other operators' parameters are held constant).

\begin{lemma}
\label{thm:increasing}
A DN layer as in Prop.~\ref{thm:layerMASO} is increasing w.r.t. each of its output dimension if and only if its slope parameters are nonnegative:
\begin{align}
    S[A^{(\ell)},B^{(\ell)}](\bu+\epsilon)& \geq S[A^{(\ell)},B^{(\ell)}](\bu),\forall \epsilon \in \mathbb{R}^{D+}\nonumber \\
    &\iff [A^{(\ell)}]_{k,r,d}\geq  0,
\end{align}
strict inequalities lead to strictly increasing layer.
\end{lemma}
\begin{theorem}
A DN whose layers $\ell=2,\dots,L$ are increasing as in Lemma~\ref{thm:increasing} is globally a MASO and thus globally convex w.r.t. the input and multivoncex w.r.t. the layer parameters. 
\label{thm:big3}
\end{theorem}
\qq
Note that Theorem \ref{thm:big3} remains true even if the first layer contains negative entries and the first nonlinearity is convex but not increasing (e.g., absolute value activation function).
\begin{theorem}
A DN whose layers $\ell=1,\dots,L$ are increasing inherit the same properties as in Thm~\ref{thm:big3} and is also increasing. 
\end{theorem}

A common theme of all of the above results is that, for DNs constructed from fully connected/convolution, activation, and pooling operators of the type stated in Prop~\ref{thm:conv}--\ref{thm:pool}, the operator/layer outputs $\bz^{(\ell)}(\bx)$ are always a {\em signal-dependent (piecewise) affine function} of the input $\bx$.
(Much more on this in Section \ref{sec:template} below.)
The particular affine mapping applied to $\bx$ depends on which partition of the spline it falls in $\R^D$.
(Much more on this in Section \ref{sec:partition} below.)

The above results pertain to DNs using convex, piecewise affine operators.
DNs using non-piecewise affine operators (e.g., the sigmoid and arctan activation functions) can be approximated as an affine spline operator that is itself a composition of MASO.
We investigate this approximation in more detail below in Section \ref{sec:universality}.



\subsection{Application: CNN Affine Mapping Formula}
\label{sec:formula}
%\green{See how we can explicitly analyze a CNN}

Combining Propositions \ref{thm:conv}--\ref{thm:pool} and Theorem \ref{thm:big2} and substituting (\ref{eq:ASO}) into (\ref{eq:layers2}), we can write an explicit formula for the output of any layer
$\bz^{(\ell)}(\bx)$ of a DN in terms of the input $\bx$ for a variety of different architectures which will be the core of the next sections aiming at analyzing how such operators model their inputs.
The formula for a standard CNN (using convolution, ReLU activation, max-pooling, and a final fully connected operator) is given in  (\ref{eq:CNNaffine}).
We derive this formula in Appendix~\ref{sec:sm_CNN}.

%and analogous formulas for resnets (see Section \ref{sec:resnet}) and RNNs (see Appendix \ref{sec:sm_RNN}) in the SM.


In (\ref{eq:CNNaffine}), 
$A^{(\ell)}_{\sigma}[\bx]$ are the signal-dependent matrices corresponding to the ReLu activation functions, 
$A_{\rho}^{(\ell)}[\bx]$ are the signal-dependent matrices corresponding to the max-pooling operators, and the biases $\bb_{\bW}^{(L)},\bb_{\bC}^{(\ell)}$ arise directly from the fully connected and convolution operators. Note the absence of $B^{(\ell)}_\sigma[\bx]$ and $B_\rho^{(\ell)}[\bx]$ due to the absence of bias term in the ReLU and max-pooling operators. It should also be clear that any desired DN topology can be rewritten as done in our case, and that this choice of topology (using only $1$ fully-connected layer and so on) serves as illustration.

By inspection of Eq.~(\ref{eq:CNNaffine}), it is clear that $\bz_{\rm CNN}^{(L)}(\bx)$ {\em is a signal-dependent, affine function of} $\bx$ (an affine spline operator, in fact).
Moreover, we can write
\begin{equation}
\bz_{\rm CNN}^{(L)}(\bx) = 
    \bW^{(L)} \left( A_{\rm CNN}[\bx]\,\bx +B_{\rm CNN}[\bx]\right) + \bb^{(L)}
    \label{eq:CNNaffine1}
\end{equation}
to recognize 
\begin{equation}
\bz_{\rm CNN}^{(L-1)}(\bx)=A_{\rm CNN}[\bx]\,\bx + B_{\rm CNN}[\bx]
\label{eq:CNNaffine1a}
\end{equation}
as an explicit, input-dependent, affine formula for the {\em featurization process} that aims to convert $\bx$ into a set of (hopefully) linearly separable features that are then input to a linear classifier with parameters $\bW^{(L)}$ and $\bb_{\bW}^{(L)}$.
 \roro{I dont know if the next paragraph is useful, personaly I dont care}Note that when using multiple fully-connected layers as last layers, all but the last one are incorporated into $A_{\rm CNN}[\bx]$ and $B_{\rm CNN}[\bx]$ as the class-agnostic representation of $\bx$ and only the last fully-connected corresponds by definition to the linear classifier.


Of course, the final prediction $\widehat{y}$ is formed by running $\bz_{\rm CNN}^{(L)}(\bx)$ through a softmax nonlinearity $g$, but this merely rescales its entries to create a probability distribution.
In particular, based on (\ref{eq:CNNaffine1a}),
$\bz^{(L-1)}(\bx)$ 
is the class agnostic, featurized representation of the input $\bx$. 
The same argument applies in the regression context if we suppress the softmax nonlinearity.
%We provide in the SM in Sec.~\ref{sec:sm_CNN} details about the above derivation.

Some interesting properties of CNNs can be inferred from Eq.~(\ref{eq:CNNaffine}), thanks to its explicit nature.
For example, what amounts to the matrix
\begin{equation}
    A_{\rm CNN}[\bx]=\prod_{\ell=L-1}^1 A_{\rho}^{(\ell)}[\bx] A^{(\ell)}_{\sigma}[\bx] \bC^{(\ell)}
    \label{eq:CNNmat}
\end{equation}
\roro{why not adding $B_{CNN}$ so that when reading part 5 one can directly refer to these equations}
has been probed and empirically shown to converge to the zero matrix as $L$ grows \roro{ok so here, at the same time it is useless and useful, useless coz you provide a formula and do not provide any property, so it is useful in a particular way: i give you the formula, compute your stuff and you will see that it converges to zeros under some condition, but I do not want to do it by myself. you see my point?}.
This observation has motivated skip-connections and resnets \cite{targ2016resnet}, to which we now turn.

\begin{figure*}[!t]
% ensure that we have normalsize text
\normalsize
% Store the current equation number.
%\setcounter{MYtempeqncnt}{\value{equation}}
% Set the equation number to one less than the one
% desired for the first equation here.
% The value here will have to changed if equations
% are added or removed prior to the place these
% equations are referenced in the main text.
%\setcounter{equation}{5}
% Restore the current equation number.
%\setcounter{equation}{\value{MYtempeqncnt}}
% IEEE uses as a separator
%\hrulefill
% The spacer can be tweaked to stop underfull vboxes.
%\vspace*{4pt}
\vspace*{-5mm}
%\hline
\begin{align}
\bz_{\rm RES}^{(L)}&(\bx)  = \small{\bW^{(L)}\underbrace{\left[ \prod_{\ell=L-1}^1\left(A_{\sigma}^{(\ell)}[\bx]\bC^{(\ell)}+ \bC^{(\ell)}_{\rm skip} \right) \right]}_{A_{\rm RES}[\bx]}\bx+\bW^{(L)}\underbrace{\sum_{\ell=L-1}^1\left(\prod_{i=L-1}^{\ell+1}( A_{\sigma}^{(\ell)}[\bx]\bC^{(\ell)}+ \bC^{(\ell)}_{\rm skip})\right)\left( A_{\sigma}^{(\ell)}[\bx]\bb_{\bC}^{(\ell)}+\bb_{\rm skip}^{(\ell)} \right)+\bb_{\bW}^{(L)}}_{\bb_{\rm RES}[\bx]}}
    \label{eq:CNNresnet}%\\[1mm]
%\vspace*{-9mm}
%\small
%    =&\underbrace{
%    \bW^{(L)}\prod_{\ell=L-1}^1 \bC^{(\ell)}_{\rm skip}}_{{\rm Linear}~(1)}\bx
%    +\underbrace{\bW^{(L)}\prod_{\ell=L-1}^2 \bC^{(\ell)}_{\rm skip}}_{{\rm Linear}~(2)}\underbrace{A_{\sigma}^{(1)}[\bx]\bW_{}^{(1)}}_{A^{(1)}_{\rm RES}[\bx]}\bx
%    +
%    \dots
%    +\underbrace{\bW^{(L)}}_{{\rm Linear}~(L)}\underbrace{\left(\prod_{k=L-1}^1 A_{\sigma}^{(k)}[\bx]\bW^{(k)} \right)}_{A^{(L)}_{\rm RES}[\bx]} \bx
%    +\bW^{(L)}\bb_{\rm RES}[\bx]+ \bb_{\bW}^{(L)}\label{eq:CNNresnet2}
\end{align}
%\hline 
\normalsize
\vspace*{-10mm}
\end{figure*}


\subsection{Application: Resnet Affine Mapping Formula}
\label{sec:resnet}


A resnet layer leverages a skip-connection that ``short-circuits'' a layer from its input to its output \cite{targ2016resnet}. 
We study here the simplest form of skip-connection that comprises a convolution operator followed by an activation operator in parallel with a second convolution operator (the so-called linear skip-connection) as in
\begin{align}
\bz^{(\ell)}(\bx)&= \bC^{(\ell)}_{\rm skip}\bz^{(\ell-1)}(\bx) \nonumber\\
& +A^{(\ell)}_{\sigma}[\bx]\left(\bC^{(\ell)}\bz^{(\ell-1)}(\bx)+\bb_{\bC}^{(\ell)}\right)+\bb^{(\ell)}_{\rm skip}.   \label{eq:resnet}
\end{align}
The  notation ``skip'' distinguishes the operator parameters for the skip-connection.
Such a topology results in state-of-the-art accuracy in standard image classification tasks \cite{targ2016resnet}.
Note that other types of skip-connections of more than $1$ layer can be simply formulated by addition of $\bC^{(\ell)}_{\rm skip-2}\bz^{(\ell-2)}(\bx)+\bC^{(\ell)}_{\rm skip-3}\bz^{(\ell-3)}(\bx)$ and so on.
%
Pooling in a standard resnet is accomplished via dyadic subsampling over pixel space and thus corresponds to a a simple subsampling of the rows of $\bC_{\rm skip}^{(\ell)}, A^{(\ell)}[\bx]$ and $\bb_{\rm skip}^{(\ell)}$ in (\ref{eq:resnet}). This solution is used here for clarity but addition of specific pooling or more complex layers is straightforward.
\iffalse
\begin{prop}
a skip-connection can be seen as a reparametrization of the layer of the MASO being by-passed as $\textbf{h}_k=\{ \ba_{k,r}+\textbf{e}_k,\forall k,r \}$ and $\textbf{b}'=\{b_{k,\omega_r},\forall k,r\}$.
\richb{i have no idea what this means.  you can just say this:} A skip-connection (\ref{eq:resnet}) is both a layer in the sense of Definition~\ref{def:layer}) and hence a MASO.
\end{prop}


\fi


Comparison of (\ref{eq:CNNaffine}) and (\ref{eq:CNNresnet}) reveals that CNNs and resnets both have the same overall functional form (in fact any composition of MASOs), including the featurization/linear classifier representation 
(\ref{eq:CNNaffine1}), (\ref{eq:CNNaffine1a}).
%(recall (\ref{eq:CNNaffine1}) and (\ref{eq:CNNaffine1a}).
However, in a resnet, there exists a linear path from the input to the output of any layer.
We can distribute this linear connection further based on (\ref{eq:CNNresnet}) to highlight an ensemble of model property as :
\small 
\begin{align}
&\bz^{(L)}_{\rm RES}(\bx)=\bb_{\bW}^{(L)}+\bW^{(L)}\huge(\bb_{\rm RES}[\bx]\nonumber \\
&\left.
\begin{array}{l}
    +\prod_{\ell=L-1}^1 \bC^{(\ell)}_{\rm skip}\bx\\
    +\prod_{\ell=L-1}^2 \bC^{(\ell)}_{\rm skip}A_{\sigma}^{(1)}[\bx]\bC^{(1)}\bx\\
    +\prod_{\ell=L-1}^3 \bC^{(\ell)}_{\rm skip}A_{\sigma}^{(2)}[\bx]\bC^{(2)}A_{\sigma}^{(1)}[\bx]\bC^{(1)}\bx\\
    + \dots\\
    +\prod_{\ell=L-1}^1 A_{\sigma}^{(\ell)}[\bx]\bW^{(\ell)}  \bx \huge)
    \end{array} \right\}\text{CNN Ensemble}
    \label{eq:CNNresnet2}
\end{align}
\normalsize
Thus, we can clearly see how a resnet can be interpreted as an ensemble of CNNs of all depths $\leq L$ \cite{veit2016residual} with tied weights.
Skip-connections and the resulting ensemble-of-CNN's structure prevent some of the detrimental stability behavior of very deep CNNs (large $L$) \cite{targ2016resnet}.
Indeed, the skip connections modify the matrix (\ref{eq:CNNmat}) that converges to zero with $L$ to 
$\prod_{\ell=L-1}^1\left(A_{\sigma}^{(\ell)}[\bx]\bC^{(\ell)}+ \bC^{(\ell)}_{\rm skip} \right)$, which is stabilized by the presence of $\bC^{(\ell)}_{\rm skip}$ \roro{DOPE! and even more DOPE if you proof what I said in the last comment}. %Details about derivations of the mapping formula and more in-depth expressions are provided in Appendix~\ref{sec:sm_RESNET}.


Formulas analogous to (\ref{eq:CNNaffine})--(\ref{eq:CNNresnet2}) can be derived for a large class of DNs; we include a formula for RNNs in Appendix~\ref{sec:sm_RNN}.
%of the SM.


%secondly, the overall mapping acts as an ensemble of standard CNN from (\ref{eq:CNNaffine}) with different depths and weight sharing across layers of the same levels.
%This ensemble structure has been studied in \cite{veit2016residual}, where it was demonstrated that that deep residual networks behave like ensemble of relatively shallow models.

%Such formulas for other DNs and in particular RNNs are provided in the SM.
%For the remaining of the paper, we denote as templates any input dependant affine mapping applied on the input $x$. This represents $A_{\rm CNN}[x]$ for the CNN and $A_{\rm RES}[x]$ for the resnet.

%We can see in (\ref{eq:CNNaffine}) the distributed formula such that there is the explicit affine mapping. The linear part will be considered as the template in further sections. On the other hand, Eq. \ref{eq:zCNN} provides the rewriting corresponding to the pre-processing and classification phase.

%\richb{can you explain this a bit more?  i don't get the dichotomic stuff}
%\randall{This is standard vision of ML for older guys, basically first provide a transformation (or pre-processing) such that you linearize your dataset THEN use a linear classifier to solve the task at hand. This dates back when pre-processing with like building features etc not just centering and scaling of the input ! Maybe it is not ''dichotomic'' but more like 2-step}
%Hence, as was done for decades in machine learning, the last layer is a linear classifier, and the composition of SO (or MASO) up the the previous to last layer performs pre-processing aiming at linearizing the problem at hand.
%This dichotomic vision of the overall DNN mapping has been exploited before. For example, in \cite{tang2013deep}, a SVM based penalty is added for the last layer to represent a linear classifier with maximized margins.


\subsection{Universality of MASO DNs}
\label{sec:universality}

\green{Equip MASO DN with the universal approximator tag}


The ability of certain neural networks to approximate an arbitrary functional/operator mapping has been well established \cite{cybenko1989approximation} with squashing activation function ($\sigma:\mathbb{R} \rightarrow [0,1]$). While it is clear that a convex operator can be approximated arbitrarily closely by one MASO, it might not be clear a priori if MASOs are adapted to approximate other more general operator. Yet, as discussed previously, most of current DNs use piecewise affine and globally convex activation function which are no squashing functions (being non convex) and in fact composition of MASOs. Hence, in SM~\ref{sec:proof_universality} %of the SM 
we prove how for general operator approximation, a composition of MASOs inherit a unversal approximation property.

\begin{theorem}
\label{thm:universality}
Let $f(\bx)_k$ represent the $k^{\rm th}$ output dimension of an arbitrary operator $f:\mathbb{R}^{D}\rightarrow \mathbb{R}^C$,
and let $f_\Theta(\bx)_k$ represent the $k^{\rm th}$ output dimension of a DN $f_\Theta$ with parameters $\Theta$  constructed from a composition of 2 MASOs.
Then, for some (optimal) parameters $\Theta$, one obtains an upper bound on the approximation error as
\begin{equation}
    \left\| f(\bx)_k - f_\Theta(\bx)_k \right\|_2 \leq \frac{c}{R},
\end{equation}
where $c$ is a constant characterizing the regularity of $f$ and $R$ the number of MASO regions (recall Eq.~\ref{eq:MASO}).
\end{theorem}
The previous Theorem demonstrates how $2$ MASOs are sufficient, given enough regions $R \gg 1$ to approximate arbitrary operators. While being sufficient and similar to results around universality of DNs, answering the question of why going deeper (large $L$, small $R$) as opposed to wider ($L=2$, large $R$) remains open and should be studied not from an approximation theory point of view (as any DN can memorize a finite dataset) but from a generalization perspective, as discussed in Sec. \ref{generalization} in the SM.
%\richb{would be great to bound $Q$ as a function of $L$ and width: not too deep and medium wide is better than very deep and not wide at all}
%\randall{a priori not possible easily, could be a paper on its own, dpeends heavily on the conditioning of all the Ws etc etc}
Nevertheless, this is enough to equip MASO DNs \roro{lool you killed me: for you guys, study that, for me it IS ENOUGH!! lmao - maybe change that stuff to something else lol} with the universality approximation property and also allows for the following corollary.
\begin{cor}
A DN with non-convex and/or non-piecewise affine operators can be approximated arbitrarily closely by a MASO-based DN. 
\label{cor:approxMaso}
\end{cor}
\qq
Corollary \ref{cor:approxMaso} expands the range of DNs to include sigmoid-based networks such as recurrent networks like RNNs, LSTMs, and GRUs \cite{graves2013generating,cho2014learning,chung2014empirical} which can be rewritten (not exactly) as composition of MASO operators.
\richb{good point i just thought of:  you don't have a formula for usual sigmoid RNNs in the appendix; just for ReLU RNNs that no one would use, right?}\randall{Nope, the formula in appendix is the general one with a piecewise affine approximation of sigmoid (as is used in practice)}


\subsection{MASOs Are Sufficient}

\green{infinite dimensional optimization of the activation functions leads to the optimal being MASO when penalizing TV(2)}\roro{GO UNSER!!!}


MASO nonlinearities are simple: piecewise-affine and globally convex. While it is well known in the theory of spline for function approximation that higher degree splines can significantly reduce the approximation error, we now demonstrate why for DNs, such argument might be unfit.

To study this question, consider a DN
made of compositions of affine transformations (with parameters $\theta$, such as convolution or fully-connected operator) and nonlinear activation functions $\sigma_k^{(\ell)},\forall \ell, k$ for each layer $\ell$ and output dimension $k$ of each of those layers that is constraint to belong to $BV(2)$, the infinite-dimensional space of functions of bounded second-order variation (see Appendix \ref{sec:proof_unser} for the precise definition). Such a functional space is infinite and in fact includes all functional $\sigma:\mathbb{R} \rightarrow \mathbb{R}$.
Thus, we obtain an optimization problem not just on the parameters $\Theta$ but also on the activation nonlinearities at each layer and each dimension leading to a much broader optimization problem as usually done in deep learning (for which activations are pre-imposed). Formally, given training data $(x_n,y_n)_{n=1}^N$, the usual cost function plus convex penalty term on the weights $\theta^{(\ell)}$ such as Tikhonov \cite{tikhonov2013numerical} denoted as $P^{(\ell)}$ and a term  
$P_\sigma= \sum_{\ell=1}^{L-1}\sum_{k=1}^{D^{(\ell)}}{\it TV}(D^2\sigma^{(\ell)}_k)$ 
 measuring the second-order total variation of the activation functions one obtains the problem:
\begin{align}
    \min_{\Theta,\sigma^{(\ell)}\in BV(2)} \sum_n  \mathcal{L}(y_n,f_\Theta(x_n))
+\mu\sum_\ell P^{(\ell)}(\theta^{(\ell)})
+\lambda P_\sigma
\label{eq:opti}
\end{align}
with $\lambda,\mu \in \mathbb{R}^+$ adjustable regularizer hyper parameters with constraint that $\|\theta^{(\ell)}\|=1$.


\begin{prop}
If an optimum to (\ref{eq:opti}) exists, then the optimal activation functions are piecewise-affine, convex functions, meaning that the DN is a composition of MASOs (with $R\leq N)$.
\label{thm:sufficient}
\end{prop}
\qq

The proof in Appendix~\ref{sec:proof_unser} leverages a recent result of \cite{unser2018representer}. 

The constraint of $\|\theta^{(\ell)}\|=1$ might be seen as unsuitable for DNs. However, we demonstrate with a simple argument how this constraint can be ignored when considering a DN layer. Due to the composition for each layer of the norm-constrained affine mapping and the arbitrary activation operator MASO $S[A^{(\ell)}_\sigma,B^{(\ell)}_\sigma]$, it is clear that rescaling of the affine transform parameters can be done via rescaling of $A^{(\ell)}_\sigma$. Since, the optimization is done over all mappings in $BV(2)$ such rescaling can correspond to the optimum (if it exists).

This motivates the suitability of MASO despite their a priori simplistic piecewise affine property. 
%The proof in Appendix~\ref{sec:proof_unser} leverages a recent result of \cite{unser2018representer}. 
Note that this results assumes the possibility to have a possibly very fine MASO ($R\leq N$) while ReLU and Leaky-ReLU are two examples with $R=2$. However, more general piecewise-affine, convex activation functions (hence MASO with $R\gg 2$) have been applied, e.g., in \cite{agostinelli2014learning}.

\roro{ok so overall this part, I do not know if it is really useful to be honnest, not because of its content but coz it seems a bit disconnected from the previous one, I dont know lets speak about it}

\iffalse

We now demonstrate that MASOs based DN come naturally from an infinite dimensional optimization problem. 
Let now consider the general form of a DN made of compositions of affine transforms and nonlinearities $\sigma_k^{(\ell)},\forall \ell, k$ such that those nonlinearities belong to $BV(2)$, the infinite space of function with bounded second order variation. 
\richb{the above includes activation functions but not pooling, right?  so is this really a general network?}
\randall{that is true that this theorems does not treat learning the pooling. HOWEVER I don't see why the theorem would not hold by allowing the BV functions to be $\mathbb{R}^{4}\rightarrow\mathbb{R}$ for example, thus leading to pooling type functions. The big problem with this is that then you would need to pre specify the pooling regions (this you can't learn directly)}

When one aims at minimizing the training set loss (cross-entropy for classification or mean-squared error for regression) w,r.t. the set of parameters $\Theta$ and the set of all activation functions as in  Eq.~\ref{eq:opti}, then, if the optimum exists, this optimal DN is a MASO based DN. Hence, the nonlinearities $\sigma_k^{(\ell)}$ are max-affine splines for each dimension of each layer.


Let define the space $BV$ of possible activation functions (univariate) as $BV=\{\sigma:\mathbb{R}\rightarrow \mathbb{R}:\|D^2\sigma\|_M< \infty\}$ the space of functional with bounded second order total variation. This infinite dimensional space is large enough to incorporate any function from $L_2$. One now aims at jointly optimizing the internal DN parameters $\Theta$ and the activation functions for each layer and each dimension. By introduction of a penalty term over their second order total variation $P_\sigma=(\sum_{\ell=1}^{L-1}\sum_{d=1}^{D^{(\ell)}}TV(D^2\sigma^{(\ell)}_d))$ and by considering a convex loss function as cross-entropy combined with softmax, and a finite training set of $N$ data points $(x_n,y_n)$ then
\begin{align}
    \argmin_{\Theta,\sigma^{(\ell)}\in BV,\forall l} \sum_n  \mathcal{L}(y_n,f_\Theta(x_n))
+\lambda P_\sigma 
+\mu\sum_\ell P^{(\ell)}(\theta^{(\ell)})\label{eq:opti}
\end{align}
and with $\lambda,\mu \in \mathbb{R}^+$ adjustable regularizer hyper parameters, $P^{(\ell)}$ a convex penalty term on the weights $\theta^{(\ell)}$ and normalized per layer weights, then if the optimal exists, it takes the form a activation function as defined in Eq. \ref{eq:mars} with $Q\leq N$ \cite{unser2018representer}.
One can see that this corresponds to a MASO based DN. Note that such activation functions with $R>2$ have been applied for example in \cite{agostinelli2014learning}.

\fi






==> intro.tex <==
\section{Introduction}
\label{sec:intro}

Deep learning has significantly advanced our ability to address a wide range of difficult machine learning and signal processing problems.
Today's machine learning landscape is dominated by {\em deep (neural) networks} (DNs), which are compositions of a large number of simple parameterized linear and nonlinear transformations.
An all-too-familiar story of late is that of plugging a deep network into an application as a black box, learning its parameter values using copious training data, and then significantly improving performance over more classical approaches.

Despite this empirical progress, the precise mechanisms by which deep learning works so well remain relatively poorly understood, adding an air of mystery to the entire field.
Ongoing attempts to build a rigorous mathematical framework fall roughly into five camps:
(i) probing and measuring networks to visualize their inner workings 
\cite{zeiler2014visualizing};
%,erhan2009visualizing}
(ii) analyzing their properties such as expressive power \cite{pmlr-v49-cohen16}, loss surface geometry \cite{lu2017depth, soudry2017exponentially}, nuisance management \cite{soatto2016visual}, 
sparsification \cite{papyan2017convolutional}, 
%https://arxiv.org/pdf/1607.08194
and generalization abilities;
(iii) new mathematical frameworks that share some (but not all) common features with DNs \cite{bruna2013invariant,mallat2012group,wiatowski2015mathematical};
(iv) probabilistic generative models from which specific DNs can be derived \cite{arora2013provable,patel2016probabilistic} and (v) statistical learning, information theory \cite{tishby2015deep}.

In this paper, we build a rigorous bridge between DNs and {\em approximation theory} via {\em spline functions and operators}.
\roro{Capital letters for of those names?}
We prove that a large class of DNs --- including convolutional neural networks (CNNs) \cite{lecun1998mnist}, residual networks \cite{resnet-he,targ2016resnet}, skip connection networks \cite{srivastava2015training}, fully connected networks \cite{pal1992multilayer}, recurrent neural networks (RNNs) \cite{graves2013generating}, scattering networks \cite{bruna2013invariant,anden2015joint}, inception \cite{szegedy2017inception} and more --- can be written as spline operators. 
Moreover, when these networks employ \roro{employ is not only for job related stuff in english?} current standard-practice piecewise-linear and convex nonlinearities (e.g., ReLU, max-pooling, etc.) they can be written as the composition of {\em max-affine spline operators}. Such operators will be derived based on max-affine splines \cite{magnani2009convex,hannah2013multivariate}, which have 
attractive approximation properties and ease of use such as the adaptive partitioning property.
% other nonlinearities it's as good of an approximation as you'd like
We focus on such nonlinearities here but note that our framework applies also to non-piecewise-linear nonlinearities through a standard approximation argument.

The spline connection provides a powerful portal through which to view and analyze the inner workings of a DN using tools from approximation theory and functional analysis. 
While prior works relating DNs with piecewise linear splines are present such as \cite{montufar2014number,rister2017piecewise,unser2018representer}, most of the theoretical studies were performed either on very specific topologies and configurations or with aim to provide theoretical guarantees and bounds on specific properties such as DN approximation capacities, input stability. 


We will thus propose insights and experiments on each developed point of this paper.
Most importantly, we demonstrate below in Section \ref{sec:deepMaso} that, {\em conditioned on the input signal, the output of a DN is an affine transformation of the input.}
\richb{actually, this is maybe not even the most important idea in the paper now.  update once we're finished.}\randall{yep!}
This finding has a number of immediate consequences: 
%
%\begin{itemize}

%\item 
C1: %In classification applications, %where we wish to infer the class membership of a signal, 
The affine mapping formula enables us to interpret a DN as constructing a set of {\em signal-dependent, class-specific templates} against which the signal is compared via a simple inner product. 
In Section \ref{sec:template} we relate DNs directly to the classical theory of optimal classification via matched filters and provide insights into the effects of data memorization \cite{zhang2016understanding}.

C2: The {\em partition of the input space} induced by the spline operator representation links DNs to the theory of vector quantization and $K$-means clustering and enables us to study the geometry \roro{maybe speak about Voronoi map, always better than Kmean perspective} of how a DN learns to organize and cluster signals. 
In Section \ref{sec:partition} we illustrate the utility of knowing the partitioning by developing a novel image distance metric \roro{embedding metric? maybe detail a little bit}.  We also provide tools to analyze the per layer induced partition of the input space which can be easily computed for any DN. 

C2A: \richb{maybe more on partition stuff. awesomeness.  add last.}

C3: The {\em inference} using a DN can be analytically studied. Addition of entropy regularization to this process \roro{which process? to the loss function you mean?} leads to analytical derivation of a gated \roro{why gated activation while before it was nonlinearities?} activation function heuristically found to be optimal in \cite{ramachandran2017searching}.
\richb{i'll edit this bullet a bit}

C4: We propose a new penalty for DN learning that encourages its templates to be {\em orthogonal} with each other. In Section \ref{sec:orthoTemplate}, we show that this leads to significantly improved classification performance on standard test data sets like SVHN, CIFAR10, and CIFAR100 with no change to the DN architecture. We will also demonstrate how this change prevents overfitting.

C5: \richb{any more?}\randall{hmm not as major thing I think}


%\item We derive an {\em explicit and stable inverse formula} for a DN based on the efficient back propagation algorithm. \richb{MORE}\randall{Maybe this will be out}.

%\item We employ the inverse formula to integrate unlabeled data into training; state-of-the-art semi-supervised learning results for a number of different networks result\randall{maybe this is out}.  

%\item We derive the Lipschitz constant of a DN, which controls its sensitivity to being tricked by {\em adversarial examples} \cite{goodfellow2014explaining,kurakin2016adversarial}.
%Our derivation immediately suggests a simple yet effective remedy for adversarial examples based on \dots \richb{MORE}.


%\end{itemize}



This paper is organized as follows.  
%
Since there are currently more deep learning papers published per day than a normal human can read and understand \roro{?? we are converging to a mixture of cognitive science and sociology!}, we have structured the paper as a high-level executive summary containing only the key results and theorem statements plus 
%a voluminous appendix 
several appendices in the Supplementary Material (SM) containing the rigorous mathematical set up, proofs, additional insights, and additional examples.
%
%After two sections providing the necessary background for DNs and splines in Sections \ref{sec:back} and \ref{sec:MASO}, we establish the links in Section \ref{sec:link}.  

%The Supplementary Material (SM) file contains not only proofs of the various results and very detailed background review but also a large number of additional experiments and results.  

==> orthoTemplate.tex <==
\subsection{Application: New DNs with Orthogonal Templates}
\label{sec:orthoTemplate}
\green{orthogonal template allow for better DNs, nothing theoretical, I skipped GREEN for this section cause it is very very neat and done}

\begin{figure*}[!tb]
\Centering
CIFAR100 Large CNN\\
\begin{minipage}{0.49\textwidth}
\centering
\includegraphics[width=1\textwidth]{Figs/CIFAR100_largeCNN_histo.png}
\end{minipage}
\begin{minipage}{0.49\textwidth}
\centering
\includegraphics[width=1\textwidth]{Figs/CIFAR100_largeCNN_loss.png}
\end{minipage}
\qqq
\caption{
Orthogonal templates significantly boost DN performance with no change to the architecture.
%
(Left) Classification performance of the largeCNN trained on the CIFAR100 for different values of the orthogonality penalty $\gamma$ in (\ref{eq:orthog}).
We plot the average (back dots), standard deviation (gray shade), and maximum (blue dots) of the test set accuracy over $15$ runs.
%
(Right/Top) Training set error. 
The blue curve corresponds to $\gamma=0$, and the black curve to $\gamma=1$.
(Right/Bottom) Test set accuracy over learning.
}
\label{fig:cifar100}
\end{figure*}



\begin{figure*}[!tb]
\Centering
CIFAR10 smallCNN\\
\begin{minipage}{0.49\textwidth}
\centering
\includegraphics[width=1\textwidth]{Figs/CIFAR_smallCNN_loss.png}
\end{minipage}
\begin{minipage}{0.49\textwidth}
\Centering
\includegraphics[width=1\textwidth]{Figs/CIFAR_smallCNN_histo.png}
\end{minipage}
\caption{Left:
Orthogonal templates also help at preventing overfitting. In black a standard DN training and in blue the case with  the orthogonality penalty $\gamma$ in (\ref{eq:orthog}) set to $1$. We plot the average over $15$ runs.
Right: Orthogonal templates on smallCNN topology for SVHN and CIFAR10 dataset with variation of the orthogonality penalty $\gamma$ in (\ref{eq:orthog}). We plot the average, standard deviation and maximum test set accuracy over $15$ runs.
}
\label{fig:cifarhisto}
\end{figure*}
While a DN's signal-dependent matched filter-bank (\ref{eq:CNNaffine1}) is optimized for classifying signals immersed in additive white Gaussian noise, such a statistical model is overly simplistic for most machine learning problems of interest. In practice, errors will arise not just from random noise but also from nuisance variations in the inputs such as arbitrary rotations, positions, and modalities of the objects of interest.
%In an ideal world, the DN would learn invariances to these nuisances, but this is not possible with a finite network
The effects of these nuisances are only poorly approximated as Gaussian random errors.
%ideally, we could make a histogram of the relevant distributions to show the nonGaussian statistics
Limited work has been done on filterbanks for classification in nonGaussian noise; one promising direction involves using not matched but rather {\em orthogonal} templates \cite{eldar2001orthogonal} \roro{ok maybe explain just a little bit why it will work with orthogonal template so that the guy is convinced before going into your new loss function}.
%,eldar2002orthogonal,eldar2003optimal}.  
THERE WAS THE TEMPLATE MATCHING W.R.T. THE INPUT AND NOW WE HAV TEMPLATE W.R.T. THE CLASS.

\iffalse
As we demonstrate above unconstrained optimization in the setting of iterative optimization and cross-entropy with softmax output nonlinearity leads to colinear templates. In particular the templates adapted to the input for the incorrect class should optimally be in opposite direction of the optimal template for the correct class. 
This goes in contradiction with the optimal theoretical template matching aiming at orthogonal templates for robust detection in the presence of possibly non Gaussian noise.
As such, we propose a penalty term forcing the induced templates to be ''always'' orthogonal.
\fi


\subsubsection{New Cost Function for Orthogonal Class Templates}

As discussed, the class templates are contained in the final layer weights $W^{(L)}$ applied on the input $\bz^{(L-1)}(\bx)$, the linearized input. As a result, we will now impose for this last layer weight to be orthogonal.
This weak constraint on the DN still enables the earlier layers to create a high-performance, class-agnostic, featurized representation (recall the discussion just below (\ref{eq:CNNaffine1})).
%
%In fact, as we demonstrated before, any DNN is rewritten as in Eq. \ref{eq:CNNaffine2}. Hence the representation $z^{(L-1)}(x)$is a class agnostic representation of the input $x$ then fed into the linear classifier. As a result, $W^{(L)}$ uniquely defines the per class template while $(A_{CNN}[x],b_{CNN}[x])$ is the representation template, from layer $1$ to $L-1$ aiming at linearizing the input w.r.t. the task at hand. 
%
To create orthogonal templates during learning, we propose to add to the standard (potentially regularized) cross-entropy loss function $\mathcal{L}_{\rm CE}(x,y)$ a term that penalizes non-zero off-diagonal entries in the matrix $W^{(L)}(W^{(L)})^T$
%Hence, to fit the OMF set up, we aim at imposing $W^{(L)}W^{(L)T}$ to be a diagonal matrix. Note that by construction the per class templates correspond to the row of $W^{(L)}$.
%As a result we propose a soft penalty term that can be added simply to the cross-entropy loss function as would be the case of any regularized like Tikhonov. We thus obtain
\begin{align}
    %\mathcal{L}_{OCE}(x,y)=
    \mathcal{L}_{\rm CE}(x,y)+\gamma \sum_{c_1 \not = c_2}\left|\left\langle [W^{(L)}]_{c_1,.}, [W^{(L)}]_{c_2,.}\right\rangle \right|^2.
    \label{eq:orthog}
\end{align}
The parameter $\gamma$ controls the tradeoff between cross-entropy minimization and orthogonality preservation.
Conveniently, when minimizing (\ref{eq:orthog}) via backpropagation, the orthogonal $W^{(L)}$ will induce orthogonal backpropagation updates for the different classes.

%In fact, according to the spherical softmax formulation the optimal has the form of $W^{(L)}\bz^{(L-1)}(x_n)+b^{(L)}\propto \delta_{y_n}, \forall n$. Thus the optimal should have the form with $W^{(L)}$ an orthonormal matrix, and linearly separable representations $\bz^{(L-1)}(x_n)$.
%On the other hand, the proposed method has the ability to ''interpolate'' between colinear templates coming from the softmax nonlinearity and the orthogonal ones from the spherical softmax by simple variation of $\gamma$.


\subsubsection{Improved Classification}

We now empirically demonstrate that orthogonal templates lead to significantly improved classification performances.

We conducted a range of experiments with three different conventional DN architectures -- smallCNN, largeCNN, and Resnet4-4 -- trained on three different datasets --  SVHN, CIFAR10, and CIFAR100.
Each DN employed bias units, ReLU activations, and max-pooling as well as batch-normalization prior each ReLU. 
The full experimental details are given in the SM.
For learning, we used the Adam optimizer with an exponential learning rate decay. 
All inputs were centered to zero mean and scaled to a maximum value of one. 
No further pre-processing was performed, such as ZCA whitening \cite{nam2014local}.
We assessed how the classification performance of a given DN would change as we varied the orthogonality penalty $\gamma$ in (\ref{eq:orthog}).
For each configuration of DN architecture, training dataset, learning rate, and penalty $\gamma$, we averaged over $15$ runs to estimate the average performance and standard deviation.




The results for CIFAR100 in Figure \ref{fig:cifar100} indicate that the  benefits of the orthogonality penalty emerge distinctly as soon as $\gamma>0$. For the smallCNN topology, more significant results can be witnessed in Fig. \ref{fig:cifarhisto} with SVHN and CIFAR10. While leading to high test set accuracy, we also provide in Fig. \ref{fig:cifarloss} the evolution of the loss during training as well as the test set accuracy. Two main effects can be observed. Firstly, the test set accuracy is always increasing or constant, demonstrating robustness to overfitting. The unpenalized loss leads to a DN with increasing test set accuracy until reaching a saturation point at which the accuracy decreases. Furthermore, the train set loss (the cross-entropy to be minimized) is seen to decrease slower when using the penalty term. This might be another indication of overfitting prevention, absence of a $0$ train set error.
%Increasing $\gamma$ further marginal gains becoming smaller as $\gamma$ increases away from $0$.
%In addition of this figures we provide in Fig. \ref{fig:large_loss} the evolution of the training loss and test accuracy over batches and epochs for SVHN and CIFAR10 using the largeCNN topoplogy. In Fig. \ref{fig:large_loss} is presented again for the largeCNN the evolution of $\gamma$ on the test set for CIFAR10 and SVHN.
%
In addition to improved final accuracy and generalization performance, we see that template orthogonality reduces the temptation of the DN to overfit. 
(This is is especially visible in the SM figures.) 
One explanation is that the orthogonal weights $W^{(L)}$ positively impact not only the prediction but also the backpropagation via orthogonal gradient updates with respect to each output dimension's partial derivatives \roro{great but why? add just 2 lines of arguments (you have them in mind for sure so....)}.
%
%This can be seen clearly in this setting where for the unregularized DNN with $\gamma=0$ the testing accuracy starts going down. On the other hand, the proposed method demonstrated quite similar convergence very early in training but then drives apart by constantly increasing or being stationary once reached the DNN capacity of performing template matching.
%Finally we perform the same task on CIFAR100 dataset with the largeCNN architecture. We provide the results in Fig.~\ref{fig:cifar100}. A similar experiment with a resnet is provided in the SM.



==> partition.tex <==
\section{DN's Intrinsic Multiscale Partition}
\label{sec:partition}
\green{we basically probe and explain the theoretical result of Sec 5}


\begin{figure*}[!tb]
    \centering
    DN with $45-3$ hidden units
\includegraphics[width=.99\textwidth]{Figs/relu_double_partitioning45_3.png}
%\\[-2mm]
%\centering 
%    DN with $25$ hidden units
%\includegraphics[width=.99\textwidth]{Figs/double_partitioning25.png}
\qqq
    \caption{Depiction of the partitioning induced by the MASO operator for each layer and its evolution during learning. From left to right one can see the initialization state, and the evolution of the partition after $40$ epochs for each subplot. The $4$-class task is depicted with different colors (blue,cyan,red and green). The top line corresponds to the partition induced by the first layer, the second line corresponds to the partition of the input space induced by the second layer. As can be seen, due to using here $45$ hidden units in the first layer, the regions boundaries are spread around the dataset offering the best separability for the second layer to build on. The second layer however having only $3$ neurons aggregates together many regions of the input space, based on the previously done partition of the first layer. This is how composition of MASO can learn arbitrary partitioning and is highlighted in this $2$dimensional case. As will be demonstrated in Fig.~\ref{fig:insimplepartitions} each of the regions then map each input with a separate affine spline, and thus, even though the boundary of one region lies exactly on the green class, the spline induced spline mapping remains able to separate the points and reach $98\%$ of accuracy.
}
\label{fig:simplepartitions}
\end{figure*}
%Like any spline, it is the interplay between the (affine) spline mappings and the input space partition that work the magic in a DN.


Recall from Section \ref{sec:splines} that a MASO has the attractive property that it implicitly partitions the input space $\R^D$ as a function of its slope and offset parameters.
The induced partition $\Omega$ opens up a new geometric avenue to study how a DN clusters and organizes signals in a hierarchical fashion. In this section we thus explore visualization and analysis of the properties from Sec.~\ref{sec:template}.


\subsection{DN Operators Partitions and VQ}\label{sec:DNpartition}
\green{In this section with study the MASO partitioning of the input space}
In this section we first propose to study the partitioning induced by max-affine splines of MASO operators.

A MASO at level $\ell$ directly influences the partitioning of its input  space $\R^{D^{(\ell-1)}}$ and indirectly influences the partitioning of the overall signal space $\R^D$.
\green{Partitioning illustration with ReLU, also reminding what is partition for a MASO}
Let first illustrate this with the simple case of ReLU activation.
A ReLU activation operator splits each of its input dimensions into two half-planes depending on the sign of the input in each dimension. Each of the max-affine splines have their own partitioning implicitly defined by $\bA^{(\ell)}_\sigma[k,.]$ and $\bB^{(\ell)}_\sigma[k,.]$ we denote as $\omega^{(\ell)}[k,r]$ the $r^{th}$ region of the $k^{th}$ max-affine spline. For a ReLU max-affine spline, one obtains $\omega^{(\ell)}[k,1]=\{z^{(\ell-1)} \in \mathbb{R}^{D^{(\ell)}}:[z^{(\ell-1)}]_k<0\}$ and  $\omega^{(\ell)}[k,2]=\{z^{(\ell-1)} \in \mathbb{R}^{D^{(\ell)}}:[z^{(\ell-1)}]_k\geq 0\}$ corresponding to all possible inputs such that either the $k^{th}$ dimension is either negative or nonnegative.
As detailed in the SM in Sec.~\ref{sec:sm_spline_op} the MASO partition of the input space is the intersection of all the per dimension partitions.
Each of the possible nonempty intersection of the per dimension half-spaces lead to the partition of the input space $\mathbb{R}^{D^{(\ell-1)}}$ into a combinatorially large number
(up to $2^{D^{(\ell)}}$) of regions. When using more general MASO (with $R>2$), there are up to $R^{D^{(\ell)}}$ regions which can either be finite or infinite. 
\green{See what is partitioning for max-pooling}
A max-pooling operator also partitions $\R^{D^{(\ell-1)}}$ into a combinatorially large number (up to $\#R^{D^{(\ell)}}$) of regions, where $\#R$ is the size of the pooling region.
For the max-pooling each region will depend on the position of the $\argmax$ for each output dimension. 
This per-MASO partitioning of its input space constructs an overall partitioning of the entire input space $\R^D$.
We now propose experiments to visualize such partitioning and highlight how cascade of MASOs shape, operators after operators, the input space partitioning.



\green{THe theoretical partitioning can be computed easily as follows}

We now describe how to obtain the partitioning.
One can infer which region was the input in via the variable $[t^{(\ell)}(\bx)]_{k,.}$ \roro{ok here maybe we killed the part related to the $t$ so...now maybe you can introduce the formula in this part since it makes sence as you are using it} (recall (\ref{eq:tmasoeq})). As discussed in the previous section, a MASO being a collection of max-affine splines, the collection of $\{[t^{(\ell)}(\bx)]_{k,r},k=1,\dots,K\}$ characterizes the input region belonging of the joint max-affine splines making up the MASO operator.
Concerning a composition of MASO, each MASO following another MASO will use the previous MASO output to define a new partition of its input space, in turn corresponding to a new partition of the input space. This is particularly clear in the toy example of Fig. \ref{fig:simplepartitions}. 
Note that when computing the MASO output via the max operator as defined in (\ref{eq:maffine}) one does not explicitly have access to $[t^{(\ell)}(\bx)]_{k,.}$. As a result we propose the following simple strategy to compute it explicitly a posteriori.
\begin{theorem}
\label{thm:findt}
Computing $[t^{(\ell)}(\bx)]_{k,.}$ can be done easily for any MASO as 
\begin{align}
    [t^{(\ell)}(\bx)]_{k,r}=\frac{\partial [\bz^{(\ell)}(\bx)]_k}{\partial \left(\langle \bA^{(\ell)}[k,r],\bx \rangle+\bB^{(\ell)}[k,r]\right)}
\end{align}
recall (\ref{eq:tmasoeq}).
\end{theorem}
When using a soft-MASO, the values of $[t^{(\ell)}(\bx)]_{k,.}$ must be computed explicitly a priori and there is thus direct access to them.
\green{We saw the hard partitioning via the $t$ we now tie it with VQ}

Due to this restriction of one-hot style representation, MASO finds similitude with clustering models such as  Vector Quantization (VQ) \cite{gersho2012vector}. 
VQ is a standard signal processing technique for compression and clustering in which case the input $\bz^{(\ell-1)}(\bx)$ is fully encoded by exactly one representent vector. This corresponds exactly to the above with $[t^{(\ell)}(\bx)]_{k,.}$ being a one-hot vector and $[\bz^{(\ell)}(\bx)]_k=1$. Note that VQ has been used successfully in texture synthesis \cite{wei2000fast} and image encoding \cite{nasrabadi1988image}. Each max-affine splines would thus correspond to an independent Vector Quantizers with their own set of $R$ vector representent $\{\bA^{(\ell)}[k,1],\dots,\bA^{(\ell)}[k,R]\},\forall k$. In particular we will see in Sec.~\ref{sec:clustering} how this can be leveraged to visualized clustered images for each MASO od DNs.



\subsection{Manifold Learning}
\green{highlight the precedent section visually}



\begin{figure}[!tb]
    \centering
    ReLU $45-3$
\includegraphics[width=.49\textwidth]{Figs/relu_in_double_partitioning45_3.png}\\
Leaky ReLU $45-3$
\includegraphics[width=.49\textwidth]{Figs/lrelu_in_double_partitioning45_3.png}\\
Absolute Value $45-3$
\includegraphics[width=.49\textwidth]{Figs/abs_in_double_partitioning45_3.png}
%    DN with $25$ hidden units
%\includegraphics[width=.99\textwidth]{Figs/double_partitioning25.png}
\qqq
    \caption{Depiction of the affine splines associated with each of the neuron of the second layer. Namely one can see in each subplot $k=1,2,3$ the output of $\bz^{(2)}_k(\bx)=\max \left( \sum_{d=1}^{D^{(1)}}\bW^{(2)}_{k,d}\max(\langle \bW^{(1)}_{d,.},\bx\rangle+\bb^{(1)}_k,0)+\bb^{(2)}_k,0\right)$ for $\bx \in [-2,2]^2$  (for the ReLU case). All the rows corresponds to the case with $45-3$ neurons, only the used nonlinearity changes, from top to bottom : ReLU, leaky-ReLU and absolute value. One can see explicitly how linear combination of convex max-affine splines allow to model any type of piecewise linear spline over some region with boundary here depicted with a black line (only $1$ boundary as $R^{(\ell)}=2$ for all presented activations). On the other hand, one can see how some max-affine splines are more adapted than others depending on the used activation. In particular, ones with a ''deactivated regime'' (ReLU,leaky-ReLU) seem to ease the approximation process with more regular splines as they are not ''handicaped'' by the symmetry of the absolute value. Note that due to the high number of units in the first layer $D^{(1)}=45$ the mapping might not seep piecewise linear to the naked eye.
}
\label{fig:insimplepartitions}
\end{figure}



\roro{why now its manifold learning and not partitioning?? Manifold learning usually implies a reduction of the dimension of the input to be visualized, in your case the input is 2D so now need of dimensional reduction. Tell me what you think but this title is not adapted in my opinion}
We now propose a simple $2D$ experiment in order to allow the partitioning visualization induced by composition of MASOs. 
To do so we use a DN with $L=3$, thus having two hidden layers and with $D^{(L)}=4$ as it is a $4$-class classification task. We experiment with either $D^{(1)}=\{15,25,45\}$ and  $D^{(2)}=\{2,3\}$ corresponding to the number of units (a.k.a neurons) for the first and second layer. We present the $45-3$ case in Fig.~\ref{fig:simplepartitions} while the others are in the SM in Fig.~\ref{fig:simplepartitions_extra1} and \ref{fig:simplepartitions_extra2}. In all cases we used standard batch-normalization and the training set contains $5000$ points for each of the $4$ classes lying in the domain $[-2,2]^2$ and training was done using Adam optimizer, a refined gradient descent based optimization scheme. Interestingly, as seen in Fig.~\ref{fig:simplepartitions}, there is not need  to have the boundaries of the regions between two classes. In fact, the output of the MASO is the result of mapping the given input to the affine spline associate with the region. As a result, two inputs in a same region will not have the same output unless the region associated affine spline is constant.
As a results, the green points, while lying on the boundary of the regions can still be separated from the green points simply based on how far away each one of them is w.r.t. the region boundary. This will be further illustrated in Fig.~\ref{fig:insimplepartitions}.
\iffalse
Concerning an actual DN, this process can be seen to have two regimes. The first one with the MASOs of the first layers for which the number of 
\richb{please remove all talk of "neurons" which is totally new jargon that it's too late to introduce. you should be using $z^\ell$ to explain }
neurons increases $D^{(\ell)}>D^{(\ell-1)}$ leading to finer and finer partitions. 
\richb{i don't get this -- the pictures i have seen of convnets with max pooling show the net getting narrower and narrower from the beginning to end.  where does the bottleneck grow wider?  maybe at the final linear classifier?}
Then, prior to the last layer, the final layers have reducing number of neurons $\dots D^{(L-2)}>D^{(L-1)}>D^{(L)}$. This means that the input space partition has less and less regions but those regions being formed based on the previous partitioning, those regions can have arbitrary shape and thus englobe any part of $R^D$ such that $\bz^{(L)}(\bx)$ is a representation linearly separable. 
\richb{i don't get this. but you're probably right.}
We also remind that $\bz^{(L)}(\bx)$ being the output of a MASO, each component $\bz^{(L)}_k(\bx)$ characterizes the input presence in the partition $k$ and the corresponding regions. In fact each output dimension $k$ has its own partition by definition of a MASO.


\fi

\subsection{Region Statistics and Empty Regions}
\green{Here we propose statistics on the number of regions, empty regions etc}
\begin{figure}[!tb]
    \centering
    DN with $D^{(1)}=15$ units
\includegraphics[width=.45\textwidth]{Figs/simple_statistics15.png}
\\[-2mm]
\centering 
    DN with $D^{(1)}=25$ units
\includegraphics[width=.45\textwidth]{Figs/simple_statistics25.png}
\qqq
    \caption{Depiction of the number of training points in the nonempty regions in decreasing ordering. The blue line represents those quantities at initialization while the red line is after training. On the left corresponds a DN without BN and on the right with BN. This highlights the fact that with proper weight initialization, most of the points lie in the same regions. After training, refinement allows a greater number of region with training points present, yet, the repartition remains exponentially decreasing as opposed to being uniform, what could be thought as optimal. The use of BN allows more regions to contains training points due to the internal renormalization done between the layers.
}
\label{fig:simplestatistics}
\end{figure}

\green{we provide some actual stats. on the regions for one of the DN topology}
We now provide some statistics about the regions induced by the first hidden layer, $S[\bA^{(1)},\bB^{(1)}]$. For the case of $D^{(1)}=15$, the maximum number of regions is of $2^{15}=32768$ due to the use of ReLU activation. 
However, as described in the MASO construction, only few of them represent non-empty regions and are thus visible in the Figures.
Non-empty regions concern regions in the input space with volume greater than $0$. 
In fact, $K$ max-affine splines with $R$ regions do not in general lead to a MASO with $R^K$ non-empty regions as the joint max-affine spline configurations might be undoable. An illustrative example can be made as follows. Consider $K$ max-affine splines with $R=2$ and with same parameters ($\ba^{(\ell)}_{k,r}=\ba^{(\ell)}_{k',r},\forall r,\forall k\not = k'$) then, the number of non empty regions for the induced MASO is exactly $2$ as opposed to $2^K$.
For our case, the number of non-empty regions is $30$ at initialization (prior training the DN) and $88$ after training without batch-normalization and $30$ to $104$ with batch-normalization.  We can also compute the number of regions such that there is at least one training point in it. This amounts to $26$ regions at initialization and $37$ after training without batch-normalization and $26$ to $46$ otherwise. 
Note that all those statistics have been averaged over $10$ runs.

\green{number of empty regions depend on batch-normalization}
Two main observations arise in this example. Firstly, the number of actual nonempty region is relatively small compared to to maximum number of possible regions. This means that due to the parametrization of the network, from initialization to convergence, many configurations are undoable. 
The second observation comes from the ability of batch-normalization to produce after learning a number of nonempty region greater than with a DN trained without BN. Note that more nonempty regions is synonym of finer overal partition and thus finer modeling of the DN. In particular, this holds not just for nonempty regions but also for regions containing at least a training point in it, again synonym of efficiency. To further observe this phenomena we provide in Fig. \ref{fig:simplestatistics} the exact number of training points per non empty regions for all DN settings.



\iffalse
\subsection{Application: Dataset Memorization and DN Architecture}

The problem of dataset memorization arouse recently when randomly labeled dataset have seen to be \textit{memorized} by a DN as the latter is able to have perfect training set accuracy, thus on the random labels.
By definition a DN mapping is surjective mapping. This implies that while different inputs $x_1,\dots,x_n$ can be granted the exact same output, same inputs inherit necessarily identical outputs. On the other hand, one would expect that if $x_1 \approx x_2$ are two images of the same classes with very similar representations, background, intensity and colors, then the output of the DN must be similar too hence incapacitating the possible of correctly classifying random labels on large dataset where such similar inputs are present. If no such close inputs are presents, the capacity of a DN to predict random labels should not be surprising as being a complex piecewise affine mapping, any random labeling can be approximated arbitrarily closely.
\fi









\subsection{Application: Manifold Learning and Vector Quantization}\label{sec:clustering}
\roro{This part is MUCH MORE about Manifold Learning, coz it involves dimension reduction + visualization with distance etc..}
\green{just finding close region inputs is enough, no need for the mapping !}

\begin{figure*}[!tb]
    \centering
\includegraphics[width=.99\textwidth]{Figs/CIFAR_smallCNNbn1_partitioning18.png}
\\[-2mm]
\includegraphics[width=.99\textwidth]{Figs/MNIST_smallCNNbn1_partitioning44.png} 
%\\
\includegraphics[width=.99\textwidth]{Figs/SVHN_smallCNNbn1_partitioning31.png}
\qqq
    \caption{
    Example of the partition-based distance between images in the CIFAR10 (top) and SVHN (bottom) datasets.
    In each image, we plot the target image $x$ at top-left and its 15 nearest neighbors in the partition-based distance at layer $\ell$ of a smallCNN trained without batch normalization (see the SM for the details).
    From left to right, the images display layers $\ell=1,\dots, 6$, and we see that the images become further and further in euclidean distance but closer and closer in featurized distance.
    For MNIST, the target image is ambiguous between a $8$ the true class, a $7$ and possibly a $5$ and $3$. The first layer recognizes this similarity and aggregates it with such digits. However, by going deeper, the closest digits become more and more $8$s. For SVHN, the first layer aggregates together inputs with similar colors and shape, thus being closer in euclidean distance. Going deeper demonstrate aggregation of $7$ images independently of the background color. For CIFAR10, one should notice that the car color is preserved all along the layers as opposed to the angle and position of the camera w.r.t. the car.
}
\label{fig:partitions}
\end{figure*}

\green{We can not visualize in high dimensions, but we can visualize inputs associated to same or close region (a.k.a VQ)}
Unfortunately, there is no simple formula for the final partition of the signal space $\R^D$ (intersection of the partitions generated by each layer) and visualization becomes impossible as $D$ grows.
However, one can obtain the set of inputs signals $x_n$ that fall into the same partitions at each layer of a DN.
In this section we go further by demonstrating that for standard computer vision tasks, just looking at inputs of close regions (and not their feature maps as in Fig.~\ref{fig:insimplepartitions}) is already characterizing the input image class. 
\green{Since most regions are either empty or with only 1 image in it, we have to look at the ''closest ones''}
First, we call style, different version of a same content, such as different rotations, coloring, zoomin etc. Let denote by $\bA^{(\ell)}[k,r]$ the $r^{\rm th}$ style 
of the $k^{\rm th}$ max-affine spline of the MASO. Then, detecting which style is present in the input corresponds to the maximization process of max-affine splines, we denote as the inference phase. Given an input $\bz^{(\ell-1)}(\bx)$, information about the present style is denoted as the vector $[t^{(\ell)}(\bx)]_{k,.}$ and is obtained as follows  (recall (\ref{eq:maffine})):
\begin{align}
    \bz^{(\ell)}_k=&\max_{r=1,\dots,R} \langle [\bA^{(\ell)}]_{k,r,.},\bz^{(\ell-1)}(\bx)\rangle +[\bB^{(\ell)}]_{k,r}\nonumber \\
    =&\sum_{r=1}^R [t^{(\ell)}(\bx)]_{k,r}\left( \langle [\bA^{(\ell)}]_{k,r,.},\bz^{(\ell-1)}(\bx)\rangle +[\bB^{(\ell)}]_{k,r} \right),
    \label{eq:tmaso}
\end{align}
with the style vector defined as the one-hot vector such that $[t^{(\ell)}(\bx)]_{k,r}=\Indic_{\{r=\argmax_{r=1,\dots,R}  \langle [\bA^{(\ell)}]_{k,r,.},\bz^{(\ell-1)}(\bx)\rangle +[\bB^{(\ell)}]_{k,r}\}}$.




Due to the  limited amount of training data in general, we found that most regions are either empty or contain only one single training data point.
We thus first propose a distance between two regions that will allow us to compute the nearest neighbours of a target signal w.r.t. their respective region membership. We define the distance function as
$d\!\left(t^{(\ell)}(\bx_1),t^{(\ell)}(\bx_2)\right)$
between the signals $x_1$ and $x_2$ and is explicitly defined as 
\begin{align}
    d\!\left(t^{(\ell)}(\bx_1),t^{(\ell)}(\bx_2)\right)=\frac{1}{K}\sum_{k=1}^K d([t^{(\ell)}(\bx_1)]_{k,.},[t^{(\ell)}(\bx_2)]_{k,.}),
\end{align}
with $d([t^{(\ell)}(\bx_1)]_{k,.},[t^{(\ell)}(\bx_2)]_{k,.})$ a chosen vector distance, with in mind that $[t^{(\ell)}(\bx)]_{k,.} \in \bigtriangleup_{R^{(\ell)}}$ and in particular, for standard MASO, it is a one-hot vector. We thus chose 
\begin{align}
 d([t^{(\ell)}(\bx_1)]_{k,.}&,[t^{(\ell)}(\bx_2)]_{k,.})=\nonumber \\
 &\left\{ \begin{array}{l} 0 \iff \argmax_r [t^{(\ell)}(\bx_1)]_{k,r}= \argmax_r [t^{(\ell)}(\bx_2)]_{k,4}\\ 1 \end{array} \right. .   
\end{align}
Development of more sophisticated measures such as taking into account the similarity between regions based on the parameters $\bA^{(\ell)},\bB^{(\ell)}$ is left for future work. Nevertheless, with the defined distance, one can see that $d\!\left(t^{(\ell)}(\bx_1),t^{(\ell)}(\bx_2)\right) \in [0,1]$ and is equal to $1$ if all regions of the $K$ max-affine splines of the MASO are the same, and equal $0$ if all regions are different. We also remind that for any given MASO, the proposed distance can be computed easily (recall (\ref{thm:findt})). In fact, for a ReLU MASO, computing this distance corresponds simply to counting how many entries of the layer output for $x_1$ and $x_2$ are both positive or $0$ at the same indices $k=1,\dots,D^{(\ell)}$. 
For a max-pooling MASO, this corresponds to counting how many $\argmax$ positions are the same for each of the max-pooling application (hence each $k=1,\dots,D^{(\ell)}$) for $x_1$ and $x_2$. 
\iffalse
Now we have 
\begin{align}
&d\!\left(r^{(\ell)}[z^{(\ell-1)}],r^{(\ell)}[z^{(\ell-1)}]\right)
=\nonumber \\&1-
\frac{
\sum_{c,i,j}
\Indic\left(
dz^{(\ell)}[z^{(\ell-1)}]=1
\right)
\Indic\left(
dz^{(\ell)}[z^{(\ell-1)}]=1
\right)
}
{ C^{(\ell)}I^{(\ell)}J^{(\ell)} }.
\end{align}
In fact, by definition of max-pooling there is always $C^{(\ell)}I^{(\ell)}J^{(\ell)}$ 1s inside any $dz^{(\ell)}[z^{(\ell-1)}]$. And thus we count the number of times the argmax was at the same position.

\fi
Figure \ref{fig:partitions} provides a visualization of the nearest neighbors of a test image under this partition-based distance measure. for the smallCNN topology and on CIFAR10, SVHN and MNIST. Further figures are provided in the SM in Fig.~\ref{fig:partitions_extra1},\ref{fig:partitions_extra2},\ref{fig:partitions_extra3}.

%Based on those distances we provide in Fig. \ref{fig:partitions} the preview of the per layer clustering of the inputs by considering the per layer distances given a target image. This is done on a trained smallCNN.


%\richb{SENSITIVITY OF THE PARTITION}

%\subsection{Application: To What?}
%K means
%Vector quantization
%``ImageDNA$^{\rm TM}$'' clustering


==> splines.tex <==
\section{Background on Spline Operators}
\label{sec:splines}


{\em Approximation theory} is the study of how and how well \roro{how and how...go synonym} functions can best be approximated using simpler functions \cite{powell1981approximation}.
A classical example of a simpler function is a {\em spline} $s: \R^D\rightarrow \R$ \cite{schmidhuber1994discovering}.
{\em For concreteness, we will work exclusively with affine splines in this paper (a.k.a. ``linear splines''), but our ideas generalize naturally to higher-order splines.}

Consider a {\em partition} $\Omega=\{\omega_1,\dots,\omega_R\}$ of the domain $\R^D$ and a set of local mappings from each region to $\R$ denoted
$\Phi=\{\phi_{1},\dots,\phi_{R}\}$, with $\phi_{r}(\bx):\langle [\a]_{r,.},\bx\rangle +[\b]_{r}$, where
$\a \in\R^{R\times D}$ and $\b \in \R^{R}$.\footnote
{
To make the connection between splines and DNs more immediately obvious, here $\bx$ is interpreted as a point in $\R^D$, which plays the r\^{o}le of the space of signals in the other sections.
}The notation $[\a]_{r,.}$ denotes the $r^{th}$ row of $\a$ and thus corresponds to a column vector.
Then the {\em multivariate affine spline}
\begin{align}
    s[\a,\b,\Omega](\bx)
    &= \sum_{r=1}^R 
    \left(\langle [\a]_{r,.},\bx\rangle 
    + [\b]_{r} \right)\Indic(\bx \in \omega_r) \nonumber\\
    &=: \langle \a[\bx], \bx \rangle + \b[\bx]
\label{eq:lmas}
\end{align}
has hyperplane parameters $\a$ (the ``slopes'') and $\b$ (the ``offsets'').
(Here $\Indic(\bx \in \omega_r)$ denotes the indicator function that equals $1$ when $\bx \in \omega_r$ and $0$ otherwise.)
The second line of (\ref{eq:mas}) introduces the streamlined notation $\a[\bx]=[\a]_{r,.}$ when $\bx \in \omega_r$;
the definition for $\b[\bx]$ is similar. 
Such a spline is piecewise affine and piecewise convex.
However, in general, it is neither globally affine nor globally convex unless $R=1$, a case we denote as \textit{degenerate spline} since it corresponds to an affine mapping.

\iffalse
We now define a special case of multivariate affine spline for which the projection of $x$ is performed only on some of the dimensions. The \textit{active} part of $x$ denoted as $\mathcal{A}$ is thus the collection of dimensions for which there exist at least one of the $a_{\omega_r}$ active on it. It is explicitly defined as $\mathcal{A}=\{d =1,\dots, D |  a_{\omega_r,d}=0 \forall r\}$. In this case we obtain
SUGGESTED NEW
\begin{align}
    s[\ba,\bb,\Omega,\mathcal{A}](x)
    &= \sum_{r=1}^R\left( \sum_{d\in\mathcal{A}}
    a_{r,d}x_d 
    + b_{r} \right)\Indic(x \in \omega_r)\nonumber \\
    &=\sum_{r=1}^R  
    \left(\langle [a_{r}]_{\mathcal{A}},[x]_{\mathcal{A}}\rangle 
    + b_{r} \right)\Indic(x \in \omega_r)
\label{eq:lmas}
\end{align}
OLD
\begin{align}
    s[\ba,\bb,\Omega,\mathcal{A}](x)
    &= \sum_{r=1}^R\left( \sum_{d\in\mathcal{A}}
    a_{\omega_r,d}x_d 
    + b_{\omega_r} \right)\Indic(x \in \omega_r)\nonumber \\
    &=\sum_{r=1}^R  
    \left(\langle [a_{\omega_r}]_{\mathcal{A}},[x]_{\mathcal{A}}\rangle 
    + b_{\omega_r} \right)\Indic(x \in \omega_r)
\label{eq:lmas}
\end{align}
where we introduce the $[x]_{\mathcal{A}}$ notation as a way to extract the components of $x$ at indices specified by $\mathcal{A}$. 
This notation is useful to impose constraints on the hyperplanes $\ba$, in particular, to constrain some dimension to be $0$ (namely the dimensions not in $\mathcal{A}$).
One can notice that the unconstrained case corresponds to having $\mathcal{A}=\{1,\dots,D\}$. Note that in this case it suffices to explicitly define the set of parameters for which the constraint for $d\in \mathcal{A}$.
\fi

A major complication of function approximation with splines in general is the need to jointly optimize both the spline parameters $\a, \b$ and the input domain partition $\Omega$ (the ``knots'' for a $1$D spline) \cite{bennett1985structural}. 
However, if a multivariate affine spline $s[\a,\b,\Omega](\bx)$ is constrained to be {\em globally convex}, then it can be rewritten as a {\em max-affine spline} \cite{magnani2009convex,hannah2013multivariate}.
An extremely useful feature of such a spline is that {\em it is completely determined by its parameters $\a$ and $\b$ without needing to specify the partition $\Omega$}.
%; in fact the $\ba$'s and $\bb$'s implicitly define the partition.}
Consider a multivariate affine spline as was defined in Eq.~\ref{eq:lmas} being globally convex, then one has 
\begin{align}
    s[\a,\b,\Omega](\bx)=\max_{r=1,\dots,R} \langle [\a]_{r,.}, \bx\rangle +[\b]_r\;, %, \quad \forall x.
    \label{eq:maffine}
\end{align}
note that the partition $\Omega$ is thus not needed to compute the function output, and is indeed implicitly induced by a function of the parameters $\a,\b$. As such, we now rewrite any max-affine spline simply as $s[\a,\b]$.
Changes in these parameters automatically induce a change in the partition giving max-affine splines the property of being {\em adaptive partitioning splines} \cite{magnani2009convex}. 
Such a formulation is of great benefits as during learning, the underlying input space partition can be modified simply via any strategy updating the internal parameters $\a,\b$.
Any piecewise affine and globally convex spline can be rewritten in such form.
\begin{prop}
\label{thm:masoequiv}
For all continuous functional $h\in \mathcal{C}^{0}(\mathbb{R})$ piecewise affine and globally convex, $\exists \a,\b$ s.t. $h(x)=s[\a,\b](x)$.
\end{prop}
This follows from the fact that the pointwise maximum of a collection of convex functions is convex \cite{roberts1993convex}.
Using standard approximation arguments, it is easy to show that a max-affine spline can approximate an arbitrary (nonlinear) convex function arbitrarily closely \cite{nishikawa1998accurate}.
%This result provides ways to create {\em adaptive partitioning splines} by learning the collection of hyperplanes with the mappings defined as the maximum of the hyperplane projections and biases. Note that one can also approximate a nonlinear convex function via piecewise affine convex splines making this result general. By construction of the max-affine splines, there is no partition explicitly defined as opposed to standard spline as they are inferred by the hyper-planes parameters $(\ba,\bb)$. Hence changing those coefficients directly impacts the way the partition is defined as opposed to standard affine splines where those two parameters and the input space partition are not paired. This is the property that makes max-affine splines, adaptive partitioning splines \cite{magnani2009convex}. 
%\subsection{Spline Operators}
A natural extension of a spline function is a {\em spline operator} that produces a multivariate output. 
\iffalse
We define an {\em affine spline operator} (ASO) as the concatenation of $K$ multivariate affine spline functions $\left(s[\a(k),\b(k),\Omega(k)]\right)_{k=1}^K$ as in (\ref{eq:mas}) where we denoted by $(\a(k),\b(k))$ the parameters for the $k^{th}$ spline. Due to this extra indexing over $k$, we simplify notations by stacking those parameters into the variables $A$ and $B$ such that $[A]_{k,r,.}=[\a(k)]_{r,.}$ and $[B]_{k,r}=[\b(k)]_r$, and by similar notation $\Omega^S$ contains all the $K$ partitions, accessed as $[\Omega^S]_{k,r}=\omega(k)_r$. As such, the ASO is denoted as $S[A,B,\Omega^S]$ and written as
\begin{align}
    & S\!\left[A,B,\Omega^S \right]\!(\bx)
    %= \left[ 
    %\begin{matrix}
    %s[\ba_{1},\bb_{1},\Omega_1](x)\\
    %\vdots \\
    %s[\ba_{K},\bb_{K},\Omega_K](x)
    %\end{matrix}
    %\right]
    %\nonumber\\[0mm]
    = \left[ 
    \begin{matrix}
    \langle \a(1)[\bx], \bx\rangle+\b(1)[\bx]\\
    \vdots \\
    \langle \a(K)[\bx], \bx\rangle+\b(K)[\bx]
    \end{matrix}
    \right]
    \nonumber\\[0mm]
    %&=\left[ 
    %\begin{matrix}
    %a_{1}[x]^T\\
    %\vdots \\
    %a_{K}[x]^T
    %\end{matrix}
    %\right]x+
    %\left[ 
    %\begin{matrix}
    %b_{1}[x]\\
    %\vdots \\
    %b_{K}[x]
    %\end{matrix}
    %\right]
    %\nonumber\\[2mm]
    & \quad\quad = \left[ 
    \begin{matrix}
    \a(1)[\bx]^T \\
    \vdots \\
    \a(K)[\bx]^T
    \end{matrix}
    \right]x+\left[ 
    \begin{matrix}
    \b(1)[\bx]\\
    \vdots \\
    \b(K)[\bx]
    \end{matrix}
    \right] =: A[\bx]\,\bx+B[\bx],
    \label{eq:ASO}
\end{align}
\fi
We define a {\em max-affine spline operator} (MASO), denoted by $S[A,B]:\mathbb{R}^D \rightarrow \mathbb{R}^K$ with parameters $A \in \mathbb{R}^{K \times R \times D}$ and $B\in \mathbb{R}^{K \times R}$ given by,
\begin{align}
    & S\!\left[A,B\right]\!(\bx)
    %= \left[ 
    %\begin{matrix}
    %s[\ba_{1},\bb_{1},\Omega_1](x)\\
    %\vdots \\
    %s[\ba_{K},\bb_{K},\Omega_K](x)
    %\end{matrix}
    %\right]
    %\nonumber\\[0mm]
    = \left[ 
    \begin{matrix}
    \max_{r=1,\dots,R}\langle [A]_{1,r,.}, \bx\rangle+[B]_{1,r}\\
    \vdots \\
    \max_{r=1,\dots,R}\langle [A]_{K,r,.}, \bx\rangle+[B]_{K,r}
    \end{matrix}
    \right]
    \nonumber\\[0mm]
    %&=\left[ 
    %\begin{matrix}
    %a_{1}[x]^T\\
    %\vdots \\
    %a_{K}[x]^T
    %\end{matrix}
    %\right]x+
    %\left[ 
    %\begin{matrix}
    %b_{1}[x]\\
    %\vdots \\
    %b_{K}[x]
    %\end{matrix}
    %\right]
    %\nonumber\\[2mm]
    & \quad\quad = A[\bx]\,\bx+B[\bx],
    \label{eq:MASO}
\end{align}
where the rows of the matrix $A[\bx]$ and entries of the vector $B[\bx]$ contain the transposes of the slopes and offsets that were selected at the point $\bx$, respectively. Such an operator can be considered as a concatenation of $K$ independent max-affine splines from Eq.~\ref{eq:maffine}. As such, MASOs have a max-affine property analogous to Prop.~\ref{thm:masoequiv}. Being a multivariate spline operator, a MASO can approximate arbitrarily closely any (nonlinear) operator that is convex in each output dimension. 
%
While this operator will be key to the paper development, we also consider the \textit{affine spline operator} as $S[A,B,\Omega^S]$ obtained in a similar fashion by concatenating $K$ affine splines from Eq.~\ref{eq:lmas}. Details and more general development is provided in the SM Sec.~\ref{sec:sm_spline_op}.

%(\ref{eq:maffine}).
%From the independence of the different spline components and their individual max-affine properties, we have that 
%\begin{align}
%    \sum_{k=1}^K [A[\bx]x+&B[\bx]]_k= \sum_{k=1}^K \max_{r_k}(\langle [A]_{k,r_k,.},\bx \rangle + [B]_{k,r_k})\nonumber \\
%    &=\max_{r_1,\dots,r_K} \sum_{k=1}^K (\langle [A]_{k,r_k,.},\bx \rangle + [B]_{k,r_k}).
%    \label{eq:maxmax}
%\end{align}


\richb{note that really have $R_k$ but we fix to just one $R$ for DNs; see SM.}




%As for Eq. \ref{eq:maxmax}, this comes naturally by independence of the max-affine splines, each able to approximate arbitrarily closely convex functional.

%If the MASO is composed of max-affine splines equipped with an active constraint, then we denote $S\!\left[\left(s[\ba_{k},\bb_{k},\mathcal{A}_k]\right)_{k=1}^K\right]\!$.


%For more details please refer to the appendix.

%with $\ba_k=\{a_{k,\omega_r} \in \mathbb{R}^D,r=1,\dots, R_k\}$, $\bb_k=\{b_{k,\omega_r} \in \mathbb{R},r=1,\dots, R_k\}$.
%To clarify the notation, we denote $S\!\left[\left(s[\ba_{k},\bb_{k},\Omega_k]\right)_{k=1}^K\right]\!:=S\!\left[\textbf{A},\bb,\Omega\right]\!$ with $\textbf{A}=\{a_{k,\omega_r},k=1,\dots,K,r=1,\dots,R_k\}$ and $\bb=\{b_{k,\omega_r},k=1,\dots,K,r=1,\dots,R_k\}$.
%\richb{are we stacking the $a$'s into the matrix $A$?  because the set notation does not indicate that}
%\richb{also should define what $A[x]$ is.  please do.}
%More details are in Appendix[REF].
%
%more on partition below in that section


%In the context of function and operator approximation, MASOs offer many attractive properties. 
%For instance, when regressing a (possibly nonlinear) convex function we have: first, by constraining the form of the mapping, and the induced properties on the spline mapping (convex and continuous for any parameter) the optimization becomes unconstrained w.r.t. the internal spline parameters. Secondly, adding hyperplanes will make the regression loss go arbitrarily closely to $0$.


%We can now extend the result to LSOs made of a collection of $K$ max-affine splines. We denote this case as Max-Affine Spline Operator (MASO). In fact, we can leverage results from max-affine spline functions \cite{hannah2013multivariate,magnani2009convex} to obtain the output mapping of those operators.
%\begin{prop}
%Consider a spline operator (\ref{eq:ASO}) with affine and convex spline function components $(s[\ba_k,\bb_k])_{k=1}^K$ as defined in Eq. \ref{eq:maffine}, the operator has the max-affine property; that is, 
%has the max-affine property; that is, each individual output dimension is convex and the mapping can be found via a $\max$ operator applied on the local affine mappings. In fact we have
%$S\left[\left(s[\ba_{k},\bb_{k},\Omega_k]\right)_{k=1}^K\right]$, with all internal affine multivariate splines $s[\ba_{k},\bb_{k},\Omega_k]$ being convex, we have
%\begin{align}
%S[(s[\ba_k,\bb_k])_{k=1}^K](x)=&\left[
%\begin{array}{c}\max_{r=1,\dots,R_1} a_{1,\omega_r}^Tx+b_{1,\omega_r} \\
%\vdots \\
%\max_{r=1,\dots,R_K} a_{K,\omega_r}^Tx+b_{K,\omega_r} \end{array} \right]\nonumber\\[2mm]
%=&A[x]x+b[x],
%\end{align}
%As such, the partitioning is now uniquely defined through the parameters $\{\ba_k,k=1,\dots,K\}:=\textbf{A}$ and $\{\bb_k,k=1,\dots,K\}:=\bb$ and we can simply denote the operator as
%$S\!\left[\textbf{A},\bb\right]$. Such operators are denoted as Max-Affine Spline Operators (MASOs).
%\end{prop}
%\richb{this is a key theorem to have in main text?}


